Random matrices in service of ML footprint: ternary random features with no performance loss

In this article, we investigate the spectral behavior of random features kernel matrices of the type ${\bf K} = \mathbb{E}_{{\bf w}} \left[\sigma\left({\bf w}^{\sf T}{\bf x}_i\right)\sigma\left({\bf w}^{\sf T}{\bf x}_j\right)\right]_{i,j=1}^n$, with nonlinear function $\sigma(\cdot)$, data ${\bf x}_1, \ldots, {\bf x}_n \in \mathbb{R}^p$, and random projection vector ${\bf w} \in \mathbb{R}^p$ having i.i.d. entries. In a high-dimensional setting where the number of data $n$ and their dimension $p$ are both large and comparable, we show, under a Gaussian mixture model for the data, that the eigenspectrum of ${\bf K}$ is independent of the distribution of the i.i.d.(zero-mean and unit-variance) entries of ${\bf w}$, and only depends on $\sigma(\cdot)$ via its (generalized) Gaussian moments $\mathbb{E}_{z\sim \mathcal N(0,1)}[\sigma'(z)]$ and $\mathbb{E}_{z\sim \mathcal N(0,1)}[\sigma''(z)]$. As a result, for any kernel matrix ${\bf K}$ of the form above, we propose a novel random features technique, called Ternary Random Feature (TRF), that (i) asymptotically yields the same limiting kernel as the original ${\bf K}$ in a spectral sense and (ii) can be computed and stored much more efficiently, by wisely tuning (in a data-dependent manner) the function $\sigma$ and the random vector ${\bf w}$, both taking values in $\{-1,0,1\}$. The computation of the proposed random features requires no multiplication, and a factor of $b$ times less bits for storage compared to classical random features such as random Fourier features, with $b$ the number of bits to store full precision values. Besides, it appears in our experiments on real data that the substantial gains in computation and storage are accompanied with somewhat improved performances compared to state-of-the-art random features compression/quantization methods.

==> eigenvectorK2_gauss.tex <==
\addplot[mark=none,color=blue] coordinates{(0,-0.030212341404339538)(1,-0.03967018068679695)(2,-0.01961818071083852)(3,-0.032811964983920076)(4,-0.031799119648145656)(5,-0.03773542167784385)(6,-0.0172429138555839)(7,-0.027839577027599916)(8,-0.018061789443308208)(9,-0.04702926378110459)(10,-0.0315389138940207)(11,-0.023055609043314156)(12,-0.032509389314522)(13,-0.0182047424919409)(14,-0.013889021728267037)(15,-0.04350648176722435)(16,-0.012155929273188997)(17,-0.06069438795135476)(18,-0.010668074321045513)(19,-0.034449864525190194)(20,-0.026066482896485416)(21,-0.04270937187395292)(22,-0.03659439694578085)(23,-0.008645497496750129)(24,-0.026632915861684568)(25,-0.04834187683687335)(26,-0.03250330384692322)(27,-0.035167543493667935)(28,-0.03241791138645827)(29,-0.028335513369321424)(30,-0.03493480542417847)(31,-0.028986740511586166)(32,-0.02097882757262209)(33,-0.023546320462502927)(34,-0.03070619315075804)(35,-0.03482709944892092)(36,-0.031467084653571314)(37,-0.04049554883156484)(38,-0.026360006035061296)(39,-0.015151267568967732)(40,-0.03007202487488342)(41,-0.031661602556282364)(42,-0.01514426054435092)(43,-0.03290755446528018)(44,-0.03147335948568628)(45,-0.03297194078267969)(46,-0.028936965569662465)(47,-0.03500635441361001)(48,-0.023371213899601742)(49,-0.024338258781555443)(50,-0.01747125560937991)(51,-0.03429586637781548)(52,-0.02697997391539199)(53,-0.027278109630282103)(54,-0.02422821015039941)(55,-0.02324326412810737)(56,-0.03283183571349839)(57,-0.025348459055797197)(58,-0.03525754353757724)(59,-0.03452342743987294)(60,-0.03632527979782126)(61,-0.017781988352972795)(62,-0.049091566743435344)(63,-0.020216369200039892)(64,-0.03375478115284652)(65,-0.03240562628201212)(66,-0.04370910423811031)(67,-0.03416474920731133)(68,-0.03561218924541099)(69,-0.017587522697364896)(70,-0.020310476018924738)(71,-0.01742769693145144)(72,-0.03132926175990526)(73,-0.033196898552424685)(74,-0.039230334363957876)(75,-0.014502202458180001)(76,-0.023544835130643142)(77,-0.02822558628578897)(78,-0.02285551342531041)(79,-0.05194476704339223)(80,-0.042351568329362516)(81,-0.04006161370651194)(82,-0.025500093322639937)(83,-0.02861867190766371)(84,-0.028645614167131184)(85,-0.0435039726455498)(86,-0.027893983551796293)(87,-0.030975351363886832)(88,-0.025944178391665525)(89,-0.0417032530116376)(90,-0.03285034589241023)(91,-0.01859556373478761)(92,-0.04214975783193366)(93,-0.01715419273148868)(94,-0.010836824910225184)(95,-0.02840091516475239)(96,-0.02758373488916135)(97,-0.025472595336241376)(98,-0.027109870396741495)(99,-0.029426490234407895)(100,-0.020191077321777447)(101,-0.024349733408081924)(102,-0.04212750835642708)(103,-0.024142278624310537)(104,-0.04290929271260096)(105,-0.03440666344341889)(106,-0.030789937585247215)(107,-0.01820255437349527)(108,-0.02215546559239677)(109,-0.03721053910306196)(110,-0.021090787993098124)(111,-0.04314891516255996)(112,-0.035963264659266615)(113,-0.02724303862212224)(114,-0.00071131170616595)(115,-0.029060156409588044)(116,-0.01107278591566801)(117,-0.04333901764059868)(118,-0.01641785463035743)(119,-0.03142323239902027)(120,-0.028665393240659892)(121,-0.03338574535547482)(122,-0.04905928787567865)(123,-0.03526226890400878)(124,-0.02353019953349925)(125,-0.03873391631825188)(126,-0.04177013096401345)(127,-0.04125651177069855)(128,-0.022198953366886792)(129,-0.04183764485411275)(130,-0.05005670425457327)(131,-0.038530849538577584)(132,-0.03615796244186665)(133,-0.03443840950010037)(134,-0.025685469819564627)(135,-0.037102543108254026)(136,-0.023835441958047897)(137,-0.023331714288638766)(138,-0.033452250294242696)(139,-0.027190090892139532)(140,-0.010887951702146808)(141,-0.031452312460776344)(142,-0.023266453311151458)(143,-0.012935517087401562)(144,-0.0338283535186089)(145,-0.021182905535692867)(146,-0.03451320097937817)(147,-0.033771528549425014)(148,-0.023995625370949947)(149,-0.0209230531703997)(150,-0.02692746784015696)(151,-0.020622045069139543)(152,-0.03940998811884614)(153,-0.03135688811679849)(154,-0.01980608746945715)(155,-0.028943836980622813)(156,-0.034540316692090074)(157,-0.002482870474779581)(158,-0.02813733870274008)(159,-0.022163463831012975)(160,-0.025886247745686427)(161,-0.034254097397952654)(162,-0.03959029029231772)(163,-0.02933511270584956)(164,-0.023955238235745756)(165,-0.03339128007190038)(166,-0.019672084820495886)(167,-0.03054056437425713)(168,-0.03353245961878844)(169,-0.036673748201850175)(170,-0.04505996108596318)(171,-0.02854951343400937)(172,-0.028640486193686)(173,-0.017801975542732898)(174,-0.015792231649817065)(175,-0.04008585206402063)(176,-0.048479869231130075)(177,-0.02553473869882965)(178,-0.05196222212520078)(179,-0.039758603559881464)(180,-0.026410740118027007)(181,-0.043263101494944556)(182,-0.05343037561070501)(183,-0.028347648010780702)(184,-0.02531844097916935)(185,-0.021033868260814527)(186,-0.02242121358871627)(187,-0.03465917086684849)(188,-0.006820239372716952)(189,-0.014027185409355518)(190,-0.022266650634887475)(191,-0.030582541493673742)(192,-0.01296350613060343)(193,-0.03970706564571803)(194,-0.04498751230633778)(195,-0.021835874901608862)(196,-0.028601857088180725)(197,-0.022729472279259016)(198,-0.009946096577904233)(199,-0.015716546236107614)(200,-0.030265357730739875)(201,-0.022714085830311023)(202,-0.023419928699059123)(203,-0.03312292713915041)(204,-0.024646364765603456)(205,-0.012093478613802819)(206,-0.028873752574259337)(207,-0.038788004159152255)(208,-0.04342908640525498)(209,-0.031799428229649915)(210,-0.03564912195325618)(211,-0.03805159534827905)(212,-0.03533045681627431)(213,-0.009866778542280123)(214,-0.026801463207506485)(215,-0.03635162360825491)(216,-0.01802979670235246)(217,-0.020221116823376194)(218,-0.02973198731043541)(219,-0.04595385491582873)(220,-0.03977355559223241)(221,-0.018276862396464894)(222,-0.02305481392089711)(223,-0.03241945369513563)(224,-0.03382354934437824)(225,-0.03930291274677717)(226,-0.03218176318044557)(227,-0.025906675417901218)(228,-0.030158647997661492)(229,-0.042696394344579926)(230,-0.018173794510138137)(231,-0.023186564522720932)(232,-0.04815892413801276)(233,-0.01994963340054961)(234,-0.018833950579249043)(235,-0.0338071236165359)(236,-0.03115642314151798)(237,-0.03316494017339227)(238,-0.01764563323329827)(239,-0.01990880689695598)(240,-0.029935819330369585)(241,-0.051543242529678575)(242,-0.04330265368134051)(243,-0.033267101441316935)(244,-0.05070362084690409)(245,-0.021686841501846753)(246,-0.044411763526674794)(247,-0.036679032890405444)(248,-0.040176238217833324)(249,-0.012014264782462224)(250,-0.029074713463484485)(251,-0.010557575928628757)(252,-0.03536890041868372)(253,-0.027402808938899244)(254,-0.01257601230509298)(255,-0.015842502243841518)(256,-0.03206481095337057)(257,-0.022051577460964575)(258,-0.01849987590576996)(259,-0.04858818086276333)(260,-0.03358392266162286)(261,-0.046266570604583356)(262,-0.0334900024782763)(263,-0.04092115109577542)(264,-0.021942050810112638)(265,-0.011229446102139043)(266,-0.031945481209375716)(267,-0.028245653662407992)(268,-0.03488907222795012)(269,-0.025351073351739528)(270,-0.031186205894667387)(271,-0.036255400732773085)(272,-0.044054761793911094)(273,-0.02580621471758597)(274,-0.031007095926643854)(275,-0.024864009046150885)(276,-0.047840291420355154)(277,-0.04132452669334633)(278,-0.02911606252061472)(279,-0.04219501436119291)(280,-0.030660730278666445)(281,-0.04886541386535741)(282,-0.02785941176653495)(283,-0.022744548148184347)(284,-0.024919163422778497)(285,-0.022789923061867435)(286,-0.022922061967281877)(287,-0.025486845620719446)(288,-0.04450765240696684)(289,-0.036505141433605795)(290,-0.04094307375906682)(291,-0.025223935489186704)(292,-0.03389485264453849)(293,-0.01188571273370861)(294,-0.020221923307750432)(295,-0.019267803198091096)(296,-0.020966803572413577)(297,-0.046908389913163255)(298,-0.04537745896414445)(299,-0.02761691388910463)(300,-0.03673253104389004)(301,-0.018705299835947143)(302,-0.03316738608072859)(303,-0.03870005585422636)(304,-0.027595077539739794)(305,-0.021861463747584534)(306,-0.03675331879291956)(307,-0.0517292647803213)(308,-0.04075976429691498)(309,-0.037908419896137954)(310,-0.03107883638310467)(311,-0.043291745683513544)(312,-0.03607420804606919)(313,-0.023241949090151436)(314,-0.03254842101839721)(315,-0.0444032557815903)(316,-0.03163478928359685)(317,-0.04580524246478503)(318,-0.042849117395456326)(319,-0.029272628617360717)(320,-0.021119236198271572)(321,-0.025578405992736183)(322,-0.03242778241143805)(323,-0.021170710812668213)(324,-0.01853264353385005)(325,-0.020558402024739023)(326,-0.01251666313936168)(327,-0.04350668825711669)(328,-0.030543024147284988)(329,-0.013436537664648326)(330,-0.032452759666469884)(331,-0.011955456036995252)(332,-0.04318544862671781)(333,-0.04015116491854354)(334,-0.031648775223223465)(335,-0.03482054332220539)(336,-0.031160621898484335)(337,-0.014975521640908498)(338,-0.0065235899644125435)(339,-0.02269409926383274)(340,-0.03817883879532369)(341,-0.02768390746310501)(342,-0.02001695727645706)(343,-0.03171711330280628)(344,-0.04565621787160353)(345,-0.026832849385054997)(346,-0.015572297387936824)(347,-0.04174652633669117)(348,-0.010345597165060725)(349,-0.026340561738106297)(350,-0.040737001128692114)(351,-0.022170362458113112)(352,-0.049527527462307444)(353,-0.011258012926732432)(354,-0.043793024068144865)(355,-0.03313298521074856)(356,-0.025727875986780866)(357,-0.02464083640192293)(358,-0.03126463641314609)(359,-0.018120970308498584)(360,-0.003468769345702278)(361,-0.033936215662681124)(362,-0.0404006930698158)(363,-0.021538902948714803)(364,-0.03274080184099138)(365,-0.007837994812950798)(366,-0.02227362175846917)(367,-0.024030046538484565)(368,-0.0072867126914204225)(369,-0.03695813948509606)(370,-0.0180470259923037)(371,-0.04005618051441125)(372,-0.044457187419966245)(373,-0.024760281475777142)(374,-0.04023566346342829)(375,-0.024126107401781584)(376,-0.029263406022116207)(377,-0.02815477523375318)(378,-0.020737114774511567)(379,-0.025278603634780215)(380,-0.019210625391483063)(381,-0.047642518741635234)(382,-0.031901315553605473)(383,-0.0368134089281603)(384,-0.020007656078909)(385,-0.011867625264511664)(386,-0.023595764878338234)(387,-0.05001559436029479)(388,-0.022214687428294657)(389,-0.03056292409697393)(390,-0.040079175432696304)(391,-0.0470370699761811)(392,-0.02458499060478103)(393,-0.029948981870463742)(394,-0.02689130428226088)(395,-0.027561892879853448)(396,-0.03158215100985129)(397,-0.03172882654021769)(398,-0.02995627449673464)(399,-0.014291708265559927)(400,-0.03148472964984058)(401,-0.015424412064553514)(402,-0.028546128871477495)(403,-0.011277741021469589)(404,-0.02211729573629545)(405,-0.04525357937462677)(406,-0.03540061002200211)(407,-0.03152080613333702)(408,-0.023002067855553383)(409,-0.027755974189215327)(410,-0.03292177019025367)(411,-0.036976319138743725)(412,-0.026247146886951154)(413,-0.028201768312800784)(414,-0.03127850813657746)(415,-0.034953079778593486)(416,-0.03245144993458678)(417,-0.035741650186255414)(418,-0.03843171517243906)(419,-0.020791472142815605)(420,-0.02103595735597903)(421,-0.01479956494267971)(422,-0.027576775630896982)(423,-0.030693658745385273)(424,-0.02631664164656782)(425,-0.02481702448270449)(426,-0.021452746281748234)(427,-0.015237138552171505)(428,-0.024845174096736193)(429,-0.025995904396804513)(430,-0.02832570114548498)(431,-0.015687545749415506)(432,-0.025275550700120494)(433,-0.033308325179408425)(434,-0.03282380146740498)(435,-0.048052583369171765)(436,-0.02310764282008271)(437,-0.033832313871268636)(438,-0.028393604711043352)(439,-0.057362963146945924)(440,-0.03257704968297392)(441,-0.0432145445958072)(442,-0.013255175630524897)(443,-0.0348364355969901)(444,-0.03562242797729773)(445,-0.026039153419978783)(446,-0.04633919176917368)(447,-0.04104240732786697)(448,-0.037500277276288976)(449,-0.03463958897146031)(450,-0.03517366923509316)(451,-0.04177114640790019)(452,-0.029584025709228225)(453,0.00553708544073841)(454,-0.038529264975340524)(455,-0.05563256840585864)(456,-0.023699245360978134)(457,-0.031419671195767336)(458,-0.012016326396442005)(459,-0.008601774627455393)(460,-0.021665813913101732)(461,-0.02936619134284519)(462,-0.035010717223354186)(463,-0.012200340276456379)(464,-0.033014188592917104)(465,-0.04058550279061744)(466,-0.025211123421117025)(467,-0.04191082118591307)(468,-0.024023157966245535)(469,-0.021679452489077086)(470,-0.0299764248040941)(471,-0.026447414045951995)(472,-0.036100957344319)(473,-0.03888286200496078)(474,-0.0022182400107991895)(475,-0.05502786298930316)(476,-0.01917969958212014)(477,-0.034784662743465054)(478,-0.03952236236211913)(479,-0.026397816797431573)(480,-0.042230912736813786)(481,-0.010182475197242833)(482,-0.030926088863593812)(483,-0.01161199179529765)(484,-0.023050558737433016)(485,-0.04068313529253381)(486,-0.029870176239812224)(487,-0.02471638543972221)(488,-0.02315717528469188)(489,-0.0319473737637578)(490,-0.055105250283225146)(491,-0.030191341418484896)(492,-0.042812300825156246)(493,-0.02088059580065621)(494,-0.031177784209372367)(495,-0.01283092298376076)(496,-0.032123457899997716)(497,-0.022861828871034384)(498,-0.0238766693579469)(499,-0.011495939724016921)(500,-0.038146302521780404)(501,-0.03672566243525309)(502,-0.035671382332257175)(503,-0.02496239571718192)(504,-0.038475534238234466)(505,-0.034884121228199845)(506,-0.023023192841684036)(507,-0.04550540366635906)(508,-0.02771805994218009)(509,-0.03952495412429863)(510,-0.03936290316341355)(511,-0.031787431763437984)(512,0.026374482545076783)(513,0.029125865660842944)(514,0.023926953206692147)(515,0.01876633609187421)(516,0.03495442002687386)(517,0.027233627673896203)(518,0.014328518769487335)(519,0.03337750529646806)(520,0.02195123230126883)(521,0.03991516084545313)(522,0.03633178557594027)(523,0.043872496116044844)(524,0.041885008697763064)(525,0.02735184125321754)(526,0.024232218149096412)(527,0.026817553870259823)(528,0.028523231406922808)(529,0.019934817076079574)(530,0.032550600009205254)(531,0.03276721614775663)(532,0.02923295216659625)(533,0.025147908063903626)(534,0.040165286048506735)(535,0.02008395722311295)(536,0.023245081352878394)(537,0.028691100312868867)(538,0.03471717180861521)(539,0.036321388976310785)(540,0.033458167357719594)(541,0.0074710621777430075)(542,0.04787129251109005)(543,0.024954168593249962)(544,0.038567286850437074)(545,0.0491891424738009)(546,0.033558935483606715)(547,0.03304895399920636)(548,0.02497378134733545)(549,0.026965371108106737)(550,0.024981999691315256)(551,0.031860166265674256)(552,0.0317051658980428)(553,0.013321430511767464)(554,0.03583936208372795)(555,0.023456284835441196)(556,0.036854907355195816)(557,0.027631132551793846)(558,0.01998338786143058)(559,0.046566485420067985)(560,0.02558021314213337)(561,0.0422266723666588)(562,0.01806397817519772)(563,0.03298539349604495)(564,0.03661946579926622)(565,0.014093559594913886)(566,0.03071819422464134)(567,0.020540000007426024)(568,0.03461174709127701)(569,0.022590010684217274)(570,0.029875007976080156)(571,0.02486518856231886)(572,0.03305851537856613)(573,0.03457374162735836)(574,0.024757692223016197)(575,0.011326629114298593)(576,0.0362459436286288)(577,0.023342389735554452)(578,0.031549819160725516)(579,0.06423792162042015)(580,0.024801507360555263)(581,0.018339499325257993)(582,0.011170647165789076)(583,0.03882692630357179)(584,0.026747912959379165)(585,0.02311953231799178)(586,0.024868087717229)(587,0.022129974692795873)(588,0.030419734139692702)(589,0.006817779805408273)(590,0.04060441162764792)(591,0.02977341004953978)(592,0.014282203910982878)(593,0.03125086180338171)(594,0.049795342235087484)(595,0.007718217317835041)(596,0.03410655043816)(597,0.033738037478025264)(598,0.03093691001726964)(599,0.029236647147843277)(600,0.029473191137323346)(601,0.03769850409358169)(602,0.015199192400296092)(603,0.031963794924978896)(604,0.020263137235073562)(605,0.01682248980325209)(606,0.028905819646038316)(607,0.02790209212973856)(608,0.031204530028928652)(609,0.045331054482872134)(610,0.021969187717206715)(611,0.0310413873844229)(612,0.03760235065440621)(613,0.024002773309585772)(614,0.03558624625146117)(615,0.034008789151653625)(616,0.02411770543192503)(617,0.04866055354826625)(618,0.018530120140743095)(619,0.042792356626455655)(620,0.03387882269109066)(621,0.03921476096938861)(622,0.03136864639990971)(623,0.011298886464455668)(624,0.006120892949693878)(625,0.03594996580433321)(626,0.03635166878316664)(627,0.028271036321663032)(628,0.03227426159907341)(629,0.04088019241873703)(630,0.0408851104630307)(631,0.03588593659747453)(632,0.007414089276451119)(633,0.026065892640559658)(634,0.03815610014045604)(635,0.04047370403891739)(636,0.036725169979410124)(637,0.02287842988440859)(638,0.027070907058767774)(639,0.023581007329040213)(640,0.0352190216187199)(641,0.05539378768987137)(642,0.0365695189888925)(643,0.02138862689384072)(644,0.027698655925476656)(645,0.05423046715847924)(646,0.01403471060900197)(647,0.03696547835102092)(648,0.021692142221916195)(649,0.035038929073166046)(650,0.027005266087064814)(651,0.037098921567976104)(652,0.03639888582708376)(653,0.02132180835533767)(654,0.015787618722921216)(655,0.033586749966030775)(656,0.027145450982282063)(657,0.046622793498766336)(658,0.017458045787226432)(659,0.02230664797702101)(660,0.03795829724007606)(661,0.01862890335468965)(662,0.031220399176631643)(663,0.022817467968063148)(664,0.02960325450007061)(665,0.025035015465259998)(666,0.0362876547315735)(667,0.03685510834309311)(668,0.04065899491118363)(669,0.033520136550879466)(670,0.038058929070636724)(671,0.0219974998016835)(672,0.02150164402542506)(673,0.02631526575039511)(674,0.0343553479250329)(675,0.016638551715765372)(676,0.023492371400193588)(677,0.03821006181054403)(678,0.02456343183806797)(679,0.03576603781974188)(680,0.029604847010171003)(681,0.026725427463214723)(682,0.03899296483652859)(683,0.020556956216767588)(684,0.03742164485971368)(685,0.03476973261294639)(686,0.0443065498974488)(687,0.04088969067510024)(688,0.03729360055539663)(689,0.019223578760153754)(690,0.018557584314213043)(691,0.01774631847018196)(692,0.03261301280675403)(693,0.02900967932581757)(694,0.03459523484796568)(695,0.016206207444984022)(696,0.03149862018842727)(697,0.018231855738301016)(698,0.03083723903978422)(699,0.03749804215971081)(700,0.04803418577829876)(701,0.02739446647117663)(702,0.04117626981395028)(703,0.04242176410618305)(704,0.011373903128438386)(705,0.03120551865405571)(706,0.0298516921996623)(707,0.03302942518381261)(708,0.01659540706931795)(709,0.04511609980857769)(710,0.0347264254101137)(711,0.021272223149206366)(712,0.043276858789277416)(713,0.02314793771490449)(714,0.026419785588745737)(715,0.02543194087469375)(716,0.02915063723705179)(717,0.03366252149070642)(718,0.05604330867868445)(719,0.02956602364884013)(720,0.03314550451021425)(721,0.03523293170415082)(722,0.028539276013901927)(723,0.03872714992188321)(724,0.028817539958729887)(725,0.026799704474057807)(726,0.03790862203351736)(727,0.03241514422966611)(728,0.02749269303479443)(729,0.027962682729080184)(730,0.03103513781090634)(731,0.03436650615579501)(732,0.039646546222962493)(733,0.008653030151299968)(734,0.022727787021687637)(735,0.025818973038739815)(736,0.03501095586529192)(737,0.03827475338665553)(738,0.025681041330998088)(739,0.027144698576785423)(740,0.02207130387130349)(741,0.05071146632580573)(742,0.038131522158242795)(743,0.03495792737277499)(744,0.029758513228616612)(745,0.019810728427401517)(746,0.015384953003459304)(747,0.026772221254286768)(748,0.02857768690809957)(749,0.024379293766426807)(750,0.027251083265606747)(751,0.03219039017058209)(752,0.036064044154202085)(753,0.03255420166283609)(754,0.03605217404270476)(755,0.013727220481325023)(756,0.026164919468374154)(757,0.03010858487170233)(758,0.03358778824251256)(759,0.03234893804331624)(760,0.02977822925625972)(761,0.023933395669439857)(762,0.03856898758699185)(763,0.020341320240784475)(764,0.03678357871536732)(765,0.015450889125059085)(766,0.027380864104735128)(767,0.02767135430301579)(768,0.02935109296128765)(769,0.03069401266054214)(770,0.011735763860248471)(771,0.011667367235599331)(772,0.03534089234882131)(773,0.040381165730116006)(774,0.024374131527673072)(775,0.04045954317201317)(776,0.02890424965216981)(777,0.02017666561251835)(778,0.02187940599009368)(779,0.030298300018950494)(780,0.028951752588426253)(781,0.03277250234831106)(782,0.027418978833124608)(783,0.01424093908048011)(784,0.03761567184265468)(785,0.03481707526403647)(786,0.03141124065298816)(787,0.02111983254643677)(788,0.02172179867487849)(789,0.038776574513849915)(790,0.024380095892482002)(791,0.0450286337761897)(792,0.03258793039364568)(793,0.03148716933179481)(794,0.03712508312565842)(795,0.042974953709679846)(796,0.03190193038520246)(797,0.03413943595810966)(798,0.024834615086188585)(799,0.026187417403719892)(800,0.024652913216871287)(801,0.050381584001299544)(802,0.03855540015052201)(803,0.035271746083456325)(804,0.03380666968701106)(805,0.03118264952535834)(806,0.022466991559424127)(807,0.032655283965752444)(808,0.042374865441262205)(809,0.03155867068528421)(810,0.02733047765779145)(811,0.02787261199354796)(812,0.025512116003350818)(813,0.013151815036671054)(814,0.03110960257990333)(815,0.02938015660944706)(816,0.030096716369886874)(817,0.04255132245497659)(818,0.017222229236579695)(819,0.027620266092856484)(820,0.049314354957093756)(821,0.04205421615651842)(822,0.028022553065897248)(823,0.029482860076977882)(824,0.03750776357102496)(825,0.02371159134130411)(826,0.025931054350856228)(827,0.04320374537868773)(828,0.02495789115923972)(829,0.025897810241443952)(830,0.043891102317586556)(831,0.0197840260072348)(832,0.04394903754253471)(833,0.024174757562827394)(834,0.02436473088183713)(835,0.04170206561280345)(836,0.021812234602816522)(837,0.045513230413210384)(838,0.03440608279398337)(839,0.02498830141080944)(840,0.02334610902507458)(841,0.016568961276390803)(842,0.03670638959441575)(843,0.030288010569021424)(844,0.037499503278859696)(845,0.036450333175591286)(846,0.024232639431792994)(847,0.01983417030169218)(848,0.028343565702857298)(849,0.016120884206572872)(850,0.030592841484024934)(851,0.023772758753224394)(852,0.024800089097262647)(853,0.04096741058106804)(854,0.053974751278490954)(855,0.008977745278285279)(856,0.024797706817783573)(857,0.03545432641285903)(858,0.0435217686143811)(859,0.013768928663715709)(860,0.031139324173341646)(861,0.038152760187121514)(862,0.023744815731896962)(863,0.03688519933515068)(864,0.026111026147238297)(865,0.03746327377603023)(866,0.020368029144270227)(867,0.02726354092423647)(868,0.021952606793451113)(869,0.034076649057576944)(870,0.028236998241103192)(871,0.019434902152237407)(872,0.012667966023705261)(873,0.025611941723655423)(874,0.029501253256132016)(875,0.03638731898872371)(876,0.02719599323406137)(877,0.03163940533220384)(878,0.026947965324987614)(879,0.039743102698601804)(880,0.03543351605566337)(881,0.009172110010058302)(882,0.006459626854316244)(883,0.027930599742803045)(884,0.01419276988003471)(885,0.055430794122007625)(886,0.024665156366620256)(887,0.03155313074503713)(888,0.016861850920759505)(889,0.024042223824294964)(890,0.04043660481981508)(891,0.03233832305088687)(892,0.05596148686909295)(893,0.02061523835704429)(894,0.035217570009828884)(895,0.028297633307271718)(896,0.03143825709296238)(897,0.04683303071641595)(898,0.03538477084094626)(899,0.027987301564454576)(900,0.02871416275285831)(901,0.03654850653796271)(902,0.031122299576904832)(903,0.01882046286760549)(904,0.0356538087162518)(905,0.02688516677369446)(906,0.016653302520345987)(907,0.023953311057681247)(908,0.031211887281395675)(909,0.036782641108803735)(910,0.0303362171558572)(911,0.01928713162155535)(912,0.030721775444190882)(913,0.03509820033306754)(914,0.03612020346087728)(915,0.020107020998283234)(916,0.006688948838116989)(917,0.020949558909471797)(918,0.028035414761585803)(919,0.015555118387861252)(920,0.0399966672484663)(921,0.019724580047050095)(922,0.049301386786026344)(923,0.028219385971153987)(924,0.025378262900126364)(925,0.035411848350167696)(926,0.022587506116183063)(927,0.02189614755231312)(928,0.02423454701929449)(929,0.02748658650408124)(930,0.018495116126661826)(931,0.016752810794016994)(932,0.029547973069932298)(933,0.018783945462680203)(934,0.023902575074517898)(935,0.02326497653388545)(936,0.03752672062118198)(937,0.02005554008323807)(938,0.020586052951948895)(939,0.022172917698787313)(940,0.03563798297341972)(941,0.025502924860603914)(942,0.03695325416261292)(943,0.028889075876279563)(944,0.023543794188576214)(945,0.0376376685373864)(946,0.021231581145845547)(947,0.0363280120939408)(948,0.02244297907918949)(949,0.024445298774442098)(950,0.036733382735528085)(951,0.027846192918185374)(952,0.034686670863711376)(953,0.04221713150898692)(954,0.0241932240677678)(955,0.0427639431592112)(956,0.024516619173152343)(957,0.029298289552073937)(958,0.021655419060268185)(959,0.031179136400998744)(960,0.029774679353134437)(961,0.013963774547930904)(962,0.02574689335423202)(963,0.034330058536429814)(964,0.02431847231671392)(965,0.040081009145929034)(966,0.021095473434632504)(967,0.030068941376246067)(968,0.03757642268954382)(969,0.02288327581296533)(970,0.01635858894118571)(971,0.021858522077164298)(972,0.046757608131122584)(973,0.0400874191009867)(974,0.009388987778436528)(975,0.042684577227792106)(976,0.019803573413688717)(977,0.037908675557228905)(978,0.020148099922753196)(979,0.044086673128211865)(980,0.03502863626096364)(981,0.03459531546290117)(982,0.02961865998261481)(983,0.03560543478605643)(984,0.010486887487500748)(985,0.019928025826704575)(986,0.03247228084517077)(987,0.035600459670792846)(988,0.03982600587361673)(989,0.02403061677130025)(990,0.037113129517938145)(991,0.0256810150987427)(992,0.028041575861265027)(993,0.019660515594120215)(994,0.024222858506046406)(995,0.04232161695457389)(996,0.03997207740722064)(997,0.014524028629077234)(998,0.02412782369572859)(999,0.03872414671604559)(1000,0.03586138417412091)(1001,0.03977823742866978)(1002,0.05118597135815615)(1003,0.02603797476246043)(1004,0.027409488911751382)(1005,0.038951478268105334)(1006,0.023706725116555884)(1007,0.045803489313090966)(1008,0.021278090989775903)(1009,0.031150022478401665)(1010,0.024930084201611257)(1011,0.03924361503094285)(1012,0.025441200525233004)(1013,0.028737461820013292)(1014,0.03127956638931484)(1015,0.040016565616721754)(1016,0.034332506211676175)(1017,0.005013704956469716)(1018,0.018844648919424105)(1019,0.02218808078638765)(1020,0.036371807578860535)(1021,0.009364959344786587)(1022,0.03535940875054452)(1023,0.04429130336762284)};

==> eigenvectorK2_student.tex <==
\addplot[mark=none,color=blue] coordinates{(0,-0.045568918756438426)(1,-0.036409001560830045)(2,-0.044289153011056924)(3,-0.03604128179689523)(4,-0.024205831181288273)(5,-0.03272640661049668)(6,-0.018282432551211005)(7,-0.03085692969763374)(8,0.0063587502069408644)(9,-0.038162024059566584)(10,-0.027673545357738603)(11,-0.031606095990458875)(12,-0.026043731836792504)(13,-0.01882497027711863)(14,-0.021330654552587692)(15,-0.036171310161055736)(16,0.001834349263309123)(17,-0.020339067738048937)(18,-0.020830859839776453)(19,-0.03159530662229037)(20,-0.022599284596560115)(21,-0.028768728140768918)(22,-0.02475948285698865)(23,-0.027904985263576126)(24,-0.03201561903720355)(25,-0.022454443893779694)(26,-0.03259685819842631)(27,-0.03810899492103424)(28,-0.020778353323268016)(29,-0.02576303635200311)(30,-0.022737422320126165)(31,-0.02492451171041928)(32,-0.031595148477943806)(33,-0.02600926718116662)(34,-0.02807121646482185)(35,-0.04412364620988449)(36,-0.03243247985342674)(37,-0.03130353017074507)(38,-0.04783964983367572)(39,-0.029681623209894738)(40,-0.04507467647447006)(41,-0.03278194522981657)(42,-0.028017057411749192)(43,-0.018190613201558802)(44,-0.022513814449127027)(45,-0.033844276325042305)(46,-0.034651569782727154)(47,-0.024708867827390443)(48,-0.027511374192445155)(49,-0.033050592406344954)(50,-0.029174554162820755)(51,-0.011804351677808564)(52,-0.016221023635935073)(53,-0.04077125559817254)(54,-0.04057016412175222)(55,-0.03550176212781685)(56,-0.03742835485361711)(57,-0.050959333135145765)(58,-0.0415999690295953)(59,-0.028265131017493724)(60,-0.02555331345762082)(61,-0.02155201668538976)(62,-0.02955749561249897)(63,-0.0306851083892747)(64,-0.036823329916912895)(65,-0.03819611070631253)(66,-0.030785626102727184)(67,-0.022601912182364736)(68,-0.027087067242289473)(69,-0.024013321564634683)(70,-0.04852592117773554)(71,-0.025675764085210193)(72,-0.034100367616139854)(73,-0.02734672378530592)(74,-0.028673292279991016)(75,-0.04527725749268508)(76,-0.034816426605118946)(77,-0.024463903766851897)(78,-0.035470271002298305)(79,-0.05331459066458845)(80,-0.037458489470010535)(81,-0.04874144069211322)(82,-0.025322679915495278)(83,-0.037746754472416696)(84,-0.02389163548691985)(85,-0.03335492478817854)(86,-0.035714294011589945)(87,-0.038027338123686166)(88,-0.04043835247194453)(89,-0.015133790480714632)(90,-0.04054127560544036)(91,-0.025549016942122013)(92,-0.0299072379698414)(93,-0.024392903909771498)(94,-0.0369288491321444)(95,-0.027398228301208465)(96,-0.03536016649585599)(97,-0.020985366921341696)(98,-0.029608375383463947)(99,-0.032824021950394425)(100,-0.015477002496822738)(101,-0.016637040932839558)(102,-0.03258518919933092)(103,-0.01757525584058765)(104,-0.047453656868646735)(105,-0.014418777909691868)(106,-0.029937623232524562)(107,-0.051426555145478704)(108,-0.045029920584652966)(109,-0.02547507111779172)(110,-0.053736237768620236)(111,-0.035995871303827025)(112,-0.03845820148649839)(113,-0.031812484841013955)(114,-0.024961215534850964)(115,-0.024540836298086125)(116,-0.02995585026357224)(117,-0.018497730369971835)(118,-0.030097867120954188)(119,-0.02990247578171792)(120,-0.0314007875127944)(121,-0.013129714556114978)(122,-0.0204191027069893)(123,-0.048963984954424056)(124,-0.03853944604407099)(125,-0.04345432296553831)(126,-0.037589710039852106)(127,-0.04270655804859168)(128,-0.029973399200099605)(129,-0.013630998730919629)(130,-0.029487234038481407)(131,-0.016998747234599758)(132,-0.02568270489752037)(133,-0.019065093493620122)(134,-0.013406860890269491)(135,-0.026773446534976476)(136,-0.04159120503693617)(137,-0.03599120615259534)(138,-0.024523970454820496)(139,-0.04268079017917292)(140,-0.019889719518983055)(141,-0.027962523879971456)(142,-0.006980513346653136)(143,-0.023658969702588833)(144,-0.028803603313254385)(145,-0.017362611961925112)(146,-0.02825936459387275)(147,-0.027750185179547145)(148,-0.03475283285991478)(149,-0.03027616055694615)(150,-0.034752204243173185)(151,-0.02308568156289309)(152,-0.023661149872845)(153,-0.03059516977929488)(154,-0.029763791565005505)(155,-0.03872827840708186)(156,-0.006210089556941616)(157,-0.029985964251802753)(158,-0.02869218477754469)(159,-0.024571150155614334)(160,-0.020271381207457088)(161,-0.040073016733398394)(162,-0.05348304811329402)(163,-0.026763879313743813)(164,-0.020824371832027944)(165,-0.017826162708193597)(166,-0.01812174688304154)(167,-0.0358984216480897)(168,-0.018799763103089406)(169,-0.03247201853167847)(170,-0.028961601818460834)(171,-0.022868445304187315)(172,-0.04390697025788946)(173,-0.02867132354436812)(174,-0.0255187410070791)(175,-0.027366373300226003)(176,-0.034906349954117816)(177,-0.041002991888621325)(178,-0.03344810602870406)(179,-0.03312320430533718)(180,-0.02546777314481465)(181,-0.035025991956590945)(182,-0.0297923753180477)(183,-0.03673530326620342)(184,-0.020774168980810626)(185,-0.02198360214805842)(186,-0.031370750197509054)(187,-0.04152102506333323)(188,-0.026455636771064918)(189,-0.04509127226813841)(190,-0.021705053865554037)(191,-0.026353952700340383)(192,-0.02924554645152926)(193,-0.04025942902966442)(194,-0.04462359782351096)(195,-0.017013506222688487)(196,-0.03762049670345913)(197,-0.02753049436080319)(198,-0.02162834282505911)(199,-0.03447788498965647)(200,-0.03945282203262708)(201,-0.020661630896199584)(202,-0.03969097160750728)(203,-0.01684861696118137)(204,-0.017558162254167453)(205,-0.02790579036617747)(206,-0.010377424928549855)(207,-0.035554912321374074)(208,-0.04134769020529414)(209,-0.03171157324044259)(210,-0.04662749321710792)(211,-0.02182770095514332)(212,-0.03866451096162651)(213,-0.032892019758038085)(214,-0.029687023616280395)(215,-0.030946302719701016)(216,-0.03135496231549754)(217,-0.03448047312378404)(218,-0.038439567768564206)(219,-0.018333220646524914)(220,-0.02530999154544348)(221,-0.029155483423279175)(222,-0.04042440506475374)(223,-0.031260088713828744)(224,-0.031025152891414363)(225,-0.033253492303574585)(226,-0.01830898667338154)(227,-0.03510872261170762)(228,-0.03183307353571975)(229,-0.03191683259153464)(230,-0.020315813083449794)(231,-0.03390227684714505)(232,-0.03162468809887425)(233,-0.041630911137128156)(234,-0.03446050322077158)(235,-0.03514045802383097)(236,-0.03403541844879855)(237,-0.028936083072038096)(238,-0.02824059042018921)(239,-0.057988847058475075)(240,-0.02234454005545139)(241,-0.025108196146696217)(242,-0.0450203833148919)(243,-0.023714173403443166)(244,-0.03892861019716197)(245,-0.018073598784516667)(246,-0.03969452454228349)(247,-0.025126292986664488)(248,-0.03346624531142202)(249,-0.029562162153701475)(250,-0.026151375548001034)(251,-0.025205977360500093)(252,-0.037534797766525144)(253,-0.02231084958953935)(254,-0.019203803900279336)(255,-0.028872407919481476)(256,-0.029097322844561492)(257,-0.03970041641399188)(258,-0.025541919545426575)(259,-0.0234855332580435)(260,-0.05603209493612883)(261,-0.026277550940496632)(262,-0.03584128348814622)(263,-0.03316933402346626)(264,-0.030276618067583274)(265,-0.037793153322138805)(266,-0.04061638279313717)(267,-0.03614114184119547)(268,-0.03353388963283177)(269,-0.019478576564657384)(270,-0.03530123846660883)(271,-0.030797701090963518)(272,-0.03315716110288987)(273,-0.038002621007619274)(274,-0.025154386556283104)(275,-0.022132840282479364)(276,-0.02518118239586034)(277,-0.033674502407694984)(278,-0.0193938451376231)(279,-0.027315921494260324)(280,-0.030418568233098048)(281,-0.023517379481820533)(282,-0.026197625236314206)(283,-0.013258927497495672)(284,-0.04738957091601133)(285,-0.04577781522766897)(286,-0.0235989841083719)(287,-0.009721011523590912)(288,-0.00932696727040652)(289,-0.015805475900601263)(290,-0.04342179073411555)(291,-0.023406953496421162)(292,-0.030394405521349394)(293,-0.024643005271713356)(294,-0.007047952386547164)(295,-0.03545154364370605)(296,-0.03083106798472047)(297,-0.02299705100254744)(298,-0.021609167778758254)(299,-0.03922201570190355)(300,-0.014185919468979711)(301,-0.043305970684057914)(302,-0.02933812301971662)(303,-0.04307271043763976)(304,-0.011133550600304675)(305,-0.029571393060879428)(306,-0.025064423596999574)(307,-0.03312017407409273)(308,-0.026581282820155934)(309,-0.030852386692562444)(310,-0.052165083368006855)(311,-0.026505215250440733)(312,-0.021788997615579023)(313,-0.020585974927428027)(314,-0.046629198724391634)(315,-0.030466708197286634)(316,-0.02318191907295031)(317,-0.01712894932504264)(318,-0.03147289121515622)(319,-0.0375188472429745)(320,-0.025950948686185093)(321,-0.03802834407930536)(322,-0.030418583948829524)(323,-0.03564573907316448)(324,-0.030898256284266044)(325,-0.038146946146225956)(326,-0.0205699660209505)(327,-0.011997405889302745)(328,-0.03015917484749307)(329,-0.021964493186280985)(330,-0.04034139798121354)(331,-0.03972309995827384)(332,-0.032890835420961266)(333,-0.028615325181744353)(334,-0.020497966855788568)(335,-0.02010380912885024)(336,-0.02116650609323263)(337,-0.029718416224272928)(338,-0.021553555876917613)(339,-0.034447973253553484)(340,-0.042048428689906825)(341,-0.02362433581923011)(342,-0.028914001025294483)(343,-0.008651857985776215)(344,-0.03306995745503228)(345,-0.019877031344487636)(346,-0.029562642087680824)(347,-0.04261814695725197)(348,-0.041317637197620945)(349,-0.013860460544500769)(350,-0.04013017999420772)(351,-0.03228073193621203)(352,-0.041452570763606734)(353,-0.023953306147098518)(354,-0.03313366207949789)(355,-0.0315259894355056)(356,-0.03401161063839552)(357,-0.04059074385876291)(358,-0.04371274665226384)(359,-0.026027187711206063)(360,-0.02879432806492778)(361,-0.029199390559185325)(362,-0.012734337189670635)(363,-0.04007697779951256)(364,-0.04040861676734578)(365,-0.03985145612154416)(366,-0.03425675899632277)(367,-0.03642964185595718)(368,-0.010063632313634196)(369,-0.03378376527231745)(370,-0.051135095557306984)(371,-0.04283167275393625)(372,-0.02123588199791625)(373,-0.037691221171640525)(374,-0.03299412216521505)(375,-0.004577622430964257)(376,-0.041168461257979114)(377,-0.011015666928156559)(378,-0.028411806300538883)(379,-0.022546008901974616)(380,-0.03451569399956229)(381,-0.01663045195711409)(382,-0.0352553362333693)(383,-0.028227726243725153)(384,-0.046146748149034286)(385,-0.01599432758854352)(386,-0.029256242632687522)(387,-0.03031254234262045)(388,-0.026324039779963813)(389,-0.02432329144026819)(390,-0.037243502708288856)(391,-0.028710459113208686)(392,-0.019372388583656197)(393,-0.02168854951975812)(394,-0.026765532126991825)(395,-0.02820039038711128)(396,-0.049836371457390075)(397,-0.021679755408962685)(398,-0.03161863985729426)(399,-0.02861212948500981)(400,-0.029895388479499022)(401,-0.018714796055280484)(402,-0.0354160070821845)(403,-0.015378493494152776)(404,-0.030436469113158376)(405,-0.03165405207673643)(406,-0.027180432912978728)(407,-0.03049619399496166)(408,-0.03951608620987624)(409,-0.025197053097345774)(410,-0.032076326242629384)(411,-0.03190764138289782)(412,-0.007536004430225789)(413,-0.03829018436345141)(414,-0.04533830915142881)(415,-0.025010084986830324)(416,-0.027167498350111032)(417,-0.056190240978574155)(418,-0.04551086615469896)(419,-0.024481196801734516)(420,-0.02572712056599662)(421,-0.018609821541900946)(422,-0.042774397621646094)(423,-0.019342327288218383)(424,-0.025721424054809063)(425,-0.02150983448468925)(426,-0.04185847920904205)(427,-0.025247572826301905)(428,-0.021698956249396856)(429,-0.037530878469080084)(430,-0.022158855527425667)(431,-0.028437766195876894)(432,-0.037521371973836204)(433,-0.017874338706084767)(434,-0.029093552633016356)(435,-0.02017663763022208)(436,-0.027341762930668194)(437,-0.0396465117807248)(438,-0.027819651127901066)(439,-0.04172499046325246)(440,-0.03385301452045309)(441,-0.042371733009957155)(442,-0.010465963698564621)(443,-0.01952191532379798)(444,-0.02041330361412977)(445,-0.027546331427545406)(446,-0.010461464437582052)(447,-0.015070735393405005)(448,-0.04024402426083905)(449,-0.03742501230113054)(450,-0.023130131140361162)(451,-0.042803458729635785)(452,-0.02373444858559315)(453,-0.03183248393979888)(454,-0.03057308042765805)(455,-0.03475128297888577)(456,-0.027768449565834446)(457,-0.02838050710090352)(458,-0.052516141546005715)(459,-0.010768513997462117)(460,-0.03392760546767222)(461,-0.02544159767216662)(462,-0.022442916699852655)(463,-0.031248283782730774)(464,-0.027889381742088295)(465,-0.024180571748399028)(466,-0.03420570722801681)(467,-0.05839651427323174)(468,-0.02715086178945362)(469,-0.020880379249782904)(470,-0.020776317409665346)(471,-0.03582929057940686)(472,-0.016327813092140573)(473,-0.03685730814273036)(474,-0.030954441217296826)(475,-0.024408320590151193)(476,-0.039925877232181516)(477,-0.01877768650398988)(478,-0.02781177038719837)(479,-0.019112782111947512)(480,-0.030793921499222332)(481,-0.026194985860164388)(482,-0.02625789867316874)(483,-0.04260631730597366)(484,-0.024541133796839237)(485,-0.0325897567018971)(486,-0.028911283839364848)(487,-0.01972450025814433)(488,-0.03568737655585059)(489,-0.04185806830005889)(490,-0.016632908306082897)(491,-0.028913474328493557)(492,-0.030808032758256144)(493,-0.024796027266889224)(494,-0.02233057808297283)(495,-0.02101305264868374)(496,-0.028889861145279236)(497,-0.04281293813692236)(498,-0.05495539643027547)(499,-0.021977643917549375)(500,-0.04118965489472445)(501,-0.022465455079829996)(502,-0.034990238620299485)(503,-0.024434881473319355)(504,-0.02480883368030337)(505,-0.033833754058751775)(506,-0.02206371513750863)(507,-0.029623886966964615)(508,-0.04591927156278566)(509,-0.027027503975864734)(510,-0.023608965945707668)(511,-0.0357799068554883)(512,0.046169115516677565)(513,0.04097164903460114)(514,0.04432000963937294)(515,0.040399317040410554)(516,0.03352592237070281)(517,0.030400156070432345)(518,0.04791914156029673)(519,0.018219409309443)(520,0.02809590661462165)(521,0.026766382588121376)(522,0.03800961157325089)(523,0.03031504693708779)(524,0.04867988025193223)(525,0.03882255163154404)(526,0.016089508671117882)(527,0.03984969884415882)(528,0.02219612940979509)(529,0.014018856773003944)(530,0.035010383943155345)(531,0.019261052865022898)(532,0.0424012498632038)(533,0.028766292290606715)(534,0.027032575903018267)(535,0.03638091832496535)(536,0.03402845209975629)(537,0.02525038591732928)(538,0.02471667360443168)(539,0.02876549550204488)(540,0.007025546128810228)(541,0.017002219263493108)(542,0.038957283756938126)(543,0.021200202334611055)(544,0.035264121675521266)(545,0.033266745284260865)(546,0.027175471576632904)(547,0.02580001637522703)(548,0.03547839930305667)(549,0.02653332480023301)(550,0.029205010011481757)(551,0.03645501766253807)(552,0.03670944847914888)(553,0.020483972639139945)(554,0.034550900534431786)(555,0.04724028004267543)(556,0.01233450206991783)(557,0.031834649979503034)(558,0.043287090618216596)(559,0.040860554792578954)(560,0.03722470570222017)(561,0.02975086807182112)(562,0.048804726920896574)(563,0.03227001323832617)(564,0.033948199929741935)(565,0.034138734503394004)(566,0.053385531082073216)(567,0.01836660077583622)(568,0.03669285086420207)(569,0.028995343457941167)(570,0.03573170200360784)(571,0.01949279906823804)(572,0.027011832342650248)(573,0.03306124198791497)(574,0.031439596542849)(575,0.030385857244476934)(576,0.015683674322800708)(577,0.04876302408565572)(578,0.029482470142878688)(579,0.02867116396726717)(580,0.023439940181270772)(581,0.022559443298436718)(582,0.03539943365309441)(583,0.0350207274822156)(584,0.030799366461388738)(585,0.014202452471104719)(586,0.016227848729563617)(587,0.01731752849584025)(588,0.03905772188325535)(589,0.03195753416802079)(590,0.04022523804820255)(591,0.021940579511369084)(592,0.04319436816187778)(593,0.018231122189366417)(594,0.02973215655054533)(595,0.02686695861457891)(596,0.014660407509763692)(597,0.03660551074919054)(598,0.029375332129574234)(599,0.016455768748740197)(600,0.030956445969541602)(601,0.03193257475797681)(602,0.011280109620799525)(603,0.03306161385179865)(604,0.02254822495298916)(605,0.02472151776438913)(606,0.026898268989838284)(607,0.017341187915353443)(608,0.01856304733412102)(609,0.050009069445159995)(610,0.029565804870257822)(611,0.03829265896437307)(612,0.028626617323720648)(613,0.03789096983947092)(614,0.03063164524586229)(615,0.036165204972281456)(616,0.036623508125657206)(617,0.02565663286231727)(618,0.04818811549475885)(619,0.04529446737715982)(620,0.03440495442662681)(621,0.023912787941995466)(622,0.043920613869910786)(623,0.03278501141572083)(624,0.023683636498114613)(625,0.0358831014978265)(626,0.037279187201243194)(627,0.030447744870664508)(628,0.022601738983630534)(629,0.021731948386670898)(630,0.03643472153032617)(631,0.02940617762987558)(632,0.03342792620326117)(633,0.03987830263604256)(634,0.02747614322803842)(635,0.025259737862300406)(636,0.03396411547366158)(637,0.040379041534029735)(638,0.011236756312210747)(639,0.05059823610903382)(640,0.020858949818116826)(641,0.03278352552008604)(642,0.0202766106784097)(643,0.01837494169735034)(644,0.038824953273045776)(645,0.04792076323050904)(646,0.027531158828565137)(647,0.0356013880167659)(648,0.017034052239661)(649,0.016610555979476034)(650,0.030700804677514376)(651,0.029057539864015592)(652,0.0195520621266146)(653,0.014667814951463774)(654,0.0326521477802046)(655,0.03988593339131745)(656,0.04001524684373223)(657,0.02083455153940194)(658,0.045264848397818226)(659,0.03487941615512256)(660,0.020582733931752303)(661,0.023257689906213744)(662,0.02492564380374068)(663,0.022490237817531913)(664,0.04103121936407288)(665,0.016008568857173302)(666,0.0297056724377637)(667,0.03670068043081857)(668,0.01674191795886091)(669,0.0332201870335929)(670,0.02392079508854565)(671,0.03513688460804541)(672,0.022553390832800998)(673,0.031450409820129935)(674,0.021885389666024165)(675,0.039911759948078655)(676,0.032306884333446695)(677,0.019882522107958)(678,0.04400649820216725)(679,0.03375190511361129)(680,0.025917935426546263)(681,0.03346356107481196)(682,0.02678074677466472)(683,0.03493657741665301)(684,0.031642534153199585)(685,0.0413870438499385)(686,0.02608531577198277)(687,0.025146889700466385)(688,0.023773447854963246)(689,0.03955178386494231)(690,0.026321722991269045)(691,0.03820335935311392)(692,0.022728645292668385)(693,0.02116776117833075)(694,0.038812211593299506)(695,0.013914026640677112)(696,0.01880707089539969)(697,0.028799172377396192)(698,0.018584685179132386)(699,0.028675460579065854)(700,0.03346310872314141)(701,0.0429314819319424)(702,0.025085405846054242)(703,0.014627211567931663)(704,0.01450969119587802)(705,0.023761434238983158)(706,0.02173566505447744)(707,0.04209404235181053)(708,0.03971526497919828)(709,0.014342654567237972)(710,0.02037933717081208)(711,0.02698406350132281)(712,0.02301246462421464)(713,0.036055140380311296)(714,0.030162472757903583)(715,0.02309398327066449)(716,0.027645166382979404)(717,0.02509101708807704)(718,0.037155552280982516)(719,0.044454088542562754)(720,0.03601320512539699)(721,0.033226769964899636)(722,0.03221639052301755)(723,0.02643836827658843)(724,0.04060236339892367)(725,0.02930975779105475)(726,0.03645720583101048)(727,0.007896228972823499)(728,0.014867274995519467)(729,0.03300970961828557)(730,0.05250684855716481)(731,0.022393048460305848)(732,0.0405859401637301)(733,0.025557323946388415)(734,0.03155673770810926)(735,0.029545897134543475)(736,0.02759879658020339)(737,0.022817868217062925)(738,0.03653119350134935)(739,0.02259176662023531)(740,0.036997340515707196)(741,0.03347449078642161)(742,0.027752340982992167)(743,0.038709870891447874)(744,0.02824512182370767)(745,0.015972583690398043)(746,0.019011059951182324)(747,0.034237160163998914)(748,0.029302474783695232)(749,0.027435681173192877)(750,0.029603896069660282)(751,0.028000185696003023)(752,0.026108311968207593)(753,0.027820075025591723)(754,0.03496986222646658)(755,0.03166469049894304)(756,0.03383363470145506)(757,0.030978302120921276)(758,0.029873178817106466)(759,0.026022052722201115)(760,0.011267375353594428)(761,0.030330410218516676)(762,0.02129226178115626)(763,0.01694982892028557)(764,0.019053539794706486)(765,0.02764352599447386)(766,0.027898114062834177)(767,0.039343387213267564)(768,0.03025801243133906)(769,0.018319072835591595)(770,0.02738317975384076)(771,0.01698735419643366)(772,0.005944422880430326)(773,0.024671318334355354)(774,0.04831966461286092)(775,0.03772865151255739)(776,0.0329026791298001)(777,0.022942432201747798)(778,0.020533641077917116)(779,0.027360013768363427)(780,0.029923415599529827)(781,0.0265846409531496)(782,0.03234313614085516)(783,0.02301576834634326)(784,0.026933823076344426)(785,0.035543897276231785)(786,0.024087033992995034)(787,0.03638024853851717)(788,0.03486136918118339)(789,0.03880569569865035)(790,0.023553805293277125)(791,0.039348048904450074)(792,0.03240931133147155)(793,0.036404009235933434)(794,0.03063320078470623)(795,0.021019918716985577)(796,0.029669656563700228)(797,0.01953601057059396)(798,0.02803564978241354)(799,0.03099019110541492)(800,0.02919205563364099)(801,0.0354957981464195)(802,0.030372355575512912)(803,0.042223956855745516)(804,0.025271326224366508)(805,0.03346950813965524)(806,0.028528777395084682)(807,0.023276645556732808)(808,0.028773961400943186)(809,0.016598846985776083)(810,0.025820048741932455)(811,0.03696559354587774)(812,0.03620823237510254)(813,0.04204523394296386)(814,0.04118868857857312)(815,0.012042897761179037)(816,0.02618938807566431)(817,0.023160566025477572)(818,0.04342981931073564)(819,0.02572734227289246)(820,0.01772376519758708)(821,0.019053501730562937)(822,0.021597870629305977)(823,0.02620284304731354)(824,0.03150766357486826)(825,0.030698107415971673)(826,0.02437862655741069)(827,0.015049793548962402)(828,0.034097980008326624)(829,0.029190994627223448)(830,0.03405026644304959)(831,0.02988425208633437)(832,0.03253162530007339)(833,0.029718474579617404)(834,0.013038604765322563)(835,0.046310126148109435)(836,0.046549321101178556)(837,0.024484145111828674)(838,0.026318252437355485)(839,0.021550549090474935)(840,0.023749474571918016)(841,0.024769824134114576)(842,0.024747924298368112)(843,0.029810416028566114)(844,0.043420258201156435)(845,0.018806225810471186)(846,0.019249411435991244)(847,0.04057553309102899)(848,0.03285295613617807)(849,0.015648062800502006)(850,0.02973692844156169)(851,0.031076982472078067)(852,0.03431266692183645)(853,0.02815275374892033)(854,0.027399986035053725)(855,0.03403464031435649)(856,0.027792785377300597)(857,0.05306618125191166)(858,0.01574323222014138)(859,0.030909235922790636)(860,0.030371275178323876)(861,0.02816092551541264)(862,0.02223853787898347)(863,0.023672835253092526)(864,0.02081323127033443)(865,0.03782833388245993)(866,0.017001762699447327)(867,0.03437007189584284)(868,0.031117395758653486)(869,0.03237963793708441)(870,0.03201872978864255)(871,0.040382226262405126)(872,0.024487833757922434)(873,0.03748592034815925)(874,0.030173847670966893)(875,0.04602825582223663)(876,0.023387459574157957)(877,0.023966033810220038)(878,0.02287922451935801)(879,0.03885287973379223)(880,0.03062130262437195)(881,0.031406227392290584)(882,0.017501956357555963)(883,0.029182078840761797)(884,0.013480889706591663)(885,0.04410308595188349)(886,0.05870956861995921)(887,0.03847094945444206)(888,0.026264058902850503)(889,0.025711561451287817)(890,0.029025668337832888)(891,0.04313766839168254)(892,0.03245337078973532)(893,0.027637861270979697)(894,0.025204493054527145)(895,0.0393309789647074)(896,0.038079596840292024)(897,0.04206479250727296)(898,0.006111456144136186)(899,0.0195976671811248)(900,0.04165848685918883)(901,0.023709759806937594)(902,0.02264631720446081)(903,0.035678913784985465)(904,0.040659981573739734)(905,0.0430385880949631)(906,0.02764306631511801)(907,0.034662858392237025)(908,0.03742932632285174)(909,0.03161834530268852)(910,0.02615410014462148)(911,0.029678235819522756)(912,0.011148146017949548)(913,0.037557446649892565)(914,0.03678143167437561)(915,0.023571872122997727)(916,0.0318359206073992)(917,0.025326535801618665)(918,0.004678832127819655)(919,0.042507322103318784)(920,0.02870317817360254)(921,0.014884572074920638)(922,0.030877740727914483)(923,0.02423593702139734)(924,0.02079732695550262)(925,0.03475260576449762)(926,0.034960086627904265)(927,0.02293720981613537)(928,0.026764344079031808)(929,0.03335795172047342)(930,0.032162729171791804)(931,0.024887481244695687)(932,0.04038245629162713)(933,0.02906907537098862)(934,0.01589343268049706)(935,0.02428892298021258)(936,0.03527012180916659)(937,0.015671547632134835)(938,0.036257996426474745)(939,0.036176317730521004)(940,0.04267087484301657)(941,0.021988070202007888)(942,0.026090537011958913)(943,0.009810832278060662)(944,0.029577964369710812)(945,0.04189029079272895)(946,0.04071003869723474)(947,0.040823884597620264)(948,0.039848344930096605)(949,0.019737953575236798)(950,0.04212323405999775)(951,0.0287467636885746)(952,0.011960746778596792)(953,0.03606674583279888)(954,0.017574698913672297)(955,0.017389519729939833)(956,0.02987481643193054)(957,0.03578738328134323)(958,0.026796026439920625)(959,0.02578018942034777)(960,0.02808260189924155)(961,0.04626629168373708)(962,0.029380424094019825)(963,0.012647957721587152)(964,0.035412697259629096)(965,0.020474772890144904)(966,0.034030120640178456)(967,0.03144728362667494)(968,0.03013942304038067)(969,0.03848023342802051)(970,0.021148369532207296)(971,0.04174616477728494)(972,0.03731364722379571)(973,0.02443683220593073)(974,0.0428159168851596)(975,0.03362630384961846)(976,0.030064689428615125)(977,0.02100707643750657)(978,0.027679538122832324)(979,0.031790953586176736)(980,0.020743375404415433)(981,0.039995395249665375)(982,0.028507911257998335)(983,0.02899567541043302)(984,0.02859897573342594)(985,0.0271868175782683)(986,0.025808786787310797)(987,0.04002029187167366)(988,0.032341842157759905)(989,0.030737273891051464)(990,0.024813120017088953)(991,0.02881464617426639)(992,0.0306394056920202)(993,0.015226846517727837)(994,0.04075361921635586)(995,0.023026693406065567)(996,0.04239424614562936)(997,0.027450191276101)(998,0.040448207452140617)(999,0.03295159099855304)(1000,0.024912199922962907)(1001,0.01470645727141654)(1002,0.028402251692275733)(1003,0.024068593479055166)(1004,0.03371605047286995)(1005,0.04792857435670888)(1006,0.037908528376413786)(1007,0.018872385168308397)(1008,0.03197343502197065)(1009,0.04256795494807213)(1010,0.044885781760272206)(1011,0.03654770378628455)(1012,0.019293216228667514)(1013,0.03156584555797142)(1014,0.03689350531884999)(1015,0.026579634468849696)(1016,0.03888123100733596)(1017,0.048484594084739846)(1018,0.015043067075622122)(1019,0.03819627003331305)(1020,0.029278984810804473)(1021,0.03578989900111303)(1022,0.03301413100012674)(1023,0.03301225842858021)
};

==> figure3_m_large.tex <==
%%% on MNIST data
\begin{figure}[thb]
\centering
\begin{tabular}{cc}
  \begin{tikzpicture}[scale=.7, spy using outlines=
{circle, magnification=3, connect spies}]
  \pgfplotsset{every major grid/.style={style=densely dashed}}
\begin{axis}[no markers, legend pos = north west, xmode = log, %ymode = log, %west
        ,grid=major,xlabel={$\gamma$},ylabel={MSEs},xmin=1e-2,xmax=10000,ymin=0,ymax=1.0,     xtick={1e-2, 1e-1, 1, 100, 10000},
    xticklabels={$10^{-2}$, $10^{-1}$, $1$, $10^{2}$, $10^4$}]
\addplot[thick, magenta]coordinates{
(0.01,0.1309)(0.01778279410038923,0.13096)(0.03162277660168379,0.13095)(0.05623413251903491,0.13091)(0.1,0.1308)(0.1778279410038923,0.1307)(0.31622776601683794,0.1305)(0.5623413251903491,0.1304)(1.0,0.13048)(1.7782794100389228,0.13092429900016874)(3.1622776601683795,0.13213831044605064)(5.623413251903491,0.1347289474543393)(10.0,0.13940041013941952)(17.78279410038923,0.14689025756841414)(31.622776601683793,0.15787881523573748)(56.23413251903491,0.1729958106420982)(100.0,0.19299251095199292)(177.82794100389228,0.21916429065879424)(316.22776601683796,0.2543303089878728)(562.341325190349,0.3042532548292963)(1000.0,0.3769977603186052)(1778.2794100389228,0.4764602700258764)(3162.2776601683795,0.5936033423059992)(5623.413251903491,0.7082780385206203)(10000.0,0.8027057456274537)
};
\addplot+[thick, black, error bars/.cd, y dir=both,y explicit]coordinates{
(0.01,0.15100429939495327)+-(0.001846790598234216,0.001846790598234216)(0.01778279410038923,0.15098943630720488)+-(0.0018463784515216097,0.0018463784515216097)(0.03162277660168379,0.15096379074933725)+-(0.001845636542307494,0.001845636542307494)(0.05623413251903491,0.15092057122335506)+-(0.0018442894181843628,0.0018442894181843628)(0.1,0.15085075191804917)+-(0.0018418096942832958,0.0018418096942832958)(0.1778279410038923,0.15074636016805276)+-(0.0018371554820225768,0.0018371554820225768)(0.31622776601683794,0.15061206896243431)+-(0.0018282243573171004,0.0018282243573171004)(0.5623413251903491,0.15049192150281337)+-(0.0018108612460301075,0.0018108612460301075)(1.0,0.15051187365882784)+-(0.0017776973452353463,0.0017776973452353463)(1.7782794100389228,0.15092429900016874)+-(0.001718519931822047,0.001718519931822047)(3.1622776601683795,0.15213831044605064)+-(0.0016245108634132203,0.0016245108634132203)(5.623413251903491,0.1547289474543393)+-(0.0014939296507708256,0.0014939296507708256)(10.0,0.15940041013941952)+-(0.001331845010195067,0.001331845010195067)(17.78279410038923,0.16689025756841414)+-(0.00114534680780356,0.00114534680780356)(31.622776601683793,0.17787881523573748)+-(0.000943496630495878,0.000943496630495878)(56.23413251903491,0.1929958106420982)+-(0.0007379638456511543,0.0007379638456511543)(100.0,0.21299251095199292)+-(0.0005405741497895745,0.0005405741497895745)(177.82794100389228,0.23916429065879424)+-(0.0003874875905538485,0.0003874875905538485)(316.22776601683796,0.2743303089878728)+-(0.00040781156694131237,0.00040781156694131237)(562.341325190349,0.3242532548292963)+-(0.0006474130041337221,0.0006474130041337221)(1000.0,0.3969977603186052)+-(0.0009708886786921884,0.0009708886786921884)(1778.2794100389228,0.4964602700258764)+-(0.0012353140383805374,0.0012353140383805374)(3162.2776601683795,0.6136033423059992)+-(0.0013044009801115278,0.0013044009801115278)(5623.413251903491,0.7282780385206203)+-(0.001147842114705179,0.001147842114705179)(10000.0,0.8227057456274537)+-(0.0008670997752292802,0.0008670997752292802)
};
%%%% Ternary
\addplot+[thick, blue, error bars/.cd, y dir=both,y explicit]coordinates{(0.01,0.1930437215189061)+-(0.0023503172097623795,0.0023503172097623795)(0.01778279410038923,0.19306377245124323)+-(0.0023472141931166917,0.0023472141931166917)(0.03162277660168379,0.1930994273569296)+-(0.0023417229018409444,0.0023417229018409444)(0.05623413251903491,0.193162825642244)+-(0.0023320414110834303,0.0023320414110834303)(0.1,0.19327553465622332)+-(0.002315083777230303,0.002315083777230303)(0.1778279410038923,0.1934758042382009)+-(0.0022857171300883945,0.0022857171300883945)(0.31622776601683794,0.19383113208466995)+-(0.0022358352006149797,0.0022358352006149797)(0.5623413251903491,0.19445904156831345)+-(0.002153768096391082,0.002153768096391082)(1.0,0.19555753878159293)+-(0.0020253456063731613,0.0020253456063731613)(1.7782794100389228,0.1974372193409736)+-(0.0018384985160474604,0.0018384985160474604)(3.1622776601683795,0.20052379737624254)+-(0.0015914177384616604,0.0015914177384616604)(5.623413251903491,0.2052840840923383)+-(0.0012995529427125712,0.0012995529427125712)(10.0,0.21208117945675528)+-(0.000996390132530658,0.000996390132530658)(17.78279410038923,0.22107346821772075)+-(0.0007281460850464958,0.0007281460850464958)(31.622776601683793,0.23227612601799316)+-(0.0005402079070116743,0.0005402079070116743)(56.23413251903491,0.2457655816086592)+-(0.00045634210050101744,0.00045634210050101744)(100.0,0.26197512981080895)+-(0.000456432636516179,0.000456432636516179)(177.82794100389228,0.2822894558663279)+-(0.0004784698688671226,0.0004784698688671226)(316.22776601683796,0.31024895611771947)+-(0.00047480063737741977,0.00047480063737741977)(562.341325190349,0.3527897676062325)+-(0.00044905155775451576,0.00044905155775451576)(1000.0,0.4189892962610432)+-(0.00042662514706128196,0.00042662514706128196)(1778.2794100389228,0.5130945958314955)+-(0.0004173512393996099,0.0004173512393996099)(3162.2776601683795,0.6258410849349569)+-(0.00041170280554477445,0.00041170280554477445)(5623.413251903491,0.736847597105223)+-(0.00037671422484236353,0.00037671422484236353)(10000.0,0.8283574578221213)+-(0.0003020397967308571,0.0003020397967308571)};
\addplot+[thick, red, error bars/.cd,  y dir=both,y explicit]coordinates{(0.01,0.19454858916685963)+-(0.0021248905252814893,0.0021248905252814893)(0.01778279410038923,0.1945673362525448)+-(0.002122292637954142,0.002122292637954142)(0.03162277660168379,0.19460067823326171)+-(0.002117691155292538,0.002117691155292538)(0.05623413251903491,0.19465998150385372)+-(0.002109565759624408,0.002109565759624408)(0.1,0.19476546565958233)+-(0.002095295040149588,0.002095295040149588)(0.1778279410038923,0.1949530694496707)+-(0.0020704670232746746,0.0020704670232746746)(0.31622776601683794,0.1952864521206335)+-(0.0020279718723565814,0.0020279718723565814)(0.5623413251903491,0.19587715235778164)+-(0.0019572232995103177,0.0019572232995103177)(1.0,0.1969149797661)+-(0.0018446417838635554,0.0018446417838635554)(1.7782794100389228,0.19870210330165658)+-(0.0016775307736084865,0.0016775307736084865)(3.1622776601683795,0.20166088365785922)+-(0.0014525854400436293,0.0014525854400436293)(5.623413251903491,0.20626486642996572)+-(0.001184531180972148,0.001184531180972148)(10.0,0.2128896897255347)+-(0.0009056793927694275,0.0009056793927694275)(17.78279410038923,0.22170026428177048)+-(0.000656772419694054,0.000656772419694054)(31.622776601683793,0.2327112894418263)+-(0.00047883076203877076,0.00047883076203877076)(56.23413251903491,0.2460065661731127)+-(0.00039783804574512196,0.00039783804574512196)(100.0,0.2620444256793296)+-(0.0003979024275052686,0.0003979024275052686)(177.82794100389228,0.2822431116333787)+-(0.00045798440891488084,0.00045798440891488084)(316.22776601683796,0.31016443377745817)+-(0.0005995482561283727,0.0005995482561283727)(562.341325190349,0.3527350128161915)+-(0.000817401401369081,0.000817401401369081)(1000.0,0.418990186178295)+-(0.0010208669467430512,0.0010208669467430512)(1778.2794100389228,0.5131286194113283)+-(0.0010891165876784036,0.0010891165876784036)(3162.2776601683795,0.6258706343140414)+-(0.000976790183772484,0.000976790183772484)(5623.413251903491,0.7368566719884918)+-(0.000751071871849122,0.000751071871849122)(10000.0,0.8283519673907962)+-(0.0005140455400166863,0.0005140455400166863)};
\addplot+[thick, green, error bars/.cd, y dir=both,y explicit]coordinates{(0.01,0.19507887104061647)+-(0.0015488084361429597,0.0015488084361429597)(0.01778279410038923,0.19509603419323307)+-(0.0015473444707589789,0.0015473444707589789)(0.03162277660168379,0.19512656921267096)+-(0.0015447611939757087,0.0015447611939757087)(0.05623413251903491,0.19518091137108373)+-(0.0015402298850959323,0.0015402298850959323)(0.1,0.19527766809029007)+-(0.0015323642411138045,0.0015323642411138045)(0.1778279410038923,0.19545004387726422)+-(0.001518956601256271,0.001518956601256271)(0.31622776601683794,0.19575722792796174)+-(0.0014967997769589135,0.0014967997769589135)(0.5623413251903491,0.19630391758690757)+-(0.001462008482617432,0.001462008482617432)(1.0,0.19727067002744963)+-(0.0014115224264354485,0.0014115224264354485)(1.7782794100389228,0.19895008824923693)+-(0.001345665353062765,0.001345665353062765)(3.1622776601683795,0.20176131357056412)+-(0.0012683850262649122,0.0012683850262649122)(5.623413251903491,0.20619247056190065)+-(0.001181302859389922,0.001181302859389922)(10.0,0.21265755451838397)+-(0.001080686346650523,0.001080686346650523)(17.78279410038923,0.22136519000680996)+-(0.0009721356655344658,0.0009721356655344658)(31.622776601683793,0.2323427688306634)+-(0.0008900118296523317,0.0008900118296523317)(56.23413251903491,0.2456442419837928)+-(0.0008832315459804267,0.0008832315459804267)(100.0,0.26168450854299685)+-(0.0009541911190268868,0.0009541911190268868)(177.82794100389228,0.28185344807564205)+-(0.0010528381318129524,0.0010528381318129524)(316.22776601683796,0.30970124902037144)+-(0.0011428494823710284,0.0011428494823710284)(562.341325190349,0.35216302989926485)+-(0.00121999021457094,0.00121999021457094)(1000.0,0.41832115083727717)+-(0.0012846595482747716,0.0012846595482747716)(1778.2794100389228,0.5124447934977003)+-(0.001307015203978833,0.001307015203978833)(3162.2776601683795,0.6252800936915123)+-(0.001224422445007449,0.001224422445007449)(5623.413251903491,0.7364193896134529)+-(0.0010165672236461271,0.0010165672236461271)(10000.0,0.8280628045739906)+-(0.0007472928714454453,0.0007472928714454453)};
\coordinate (spypoint) at (axis cs:10,0.18);
\coordinate (magnifyglass) at (axis cs:10,0.5);
\legend{Baseline (KRR), RFF, $\epsilon=0.1$ (TRF), $\epsilon=0.5$ (TRF), $\epsilon=0.9$ (TRF)};
\end{axis}
\spy [blue, size=1.5cm] on (spypoint) in node[fill=white] at (magnifyglass);
\end{tikzpicture}   
& 
\begin{tikzpicture}[scale=.7]
    		\begin{axis}[legend pos = south west, %ymode = log, %west
        ,grid=major,xlabel={$\epsilon$},ylabel={Running time (s)},xmin=0.1,xmax=0.9,ymin=15,ymax=2800, xtick={0.1, 0.3, 0.5, 0.7, 0.9},
    xticklabels={$0.1$, $0.3$, $0.5$, $0.7$, $0.9$}]
     			            \addplot[mark size=4pt, magenta,  thick]coordinates{(0.1,2750)(0.5, 2750)(0.9, 2750)
};   
    			            \addplot[mark size=4pt, thick]coordinates{(0.1,1952)(0.5, 1952)(0.9, 1952)
};
    			            \addplot[mark size=4pt,red,mark=square,thick]coordinates{%(0.1,1264)(0.5, 901)(0.9, 753)
    			            (0.1,900)(0.5,846)(0.9,635)
};
\legend{KRR, RFF, TRF};
\end{axis}
\end{tikzpicture}
\end{tabular}
{\RED
\caption{Testing mean squared errors (MSEs, \textbf{LEFT}) and running time (\textbf{RIGHT}) of random features ridge regression, $p=512, n=1024, n_{test}=512, m=10^5.$ Ternary function with ${\bf W}$ distributed according to~(\ref{eq:w}) and $\epsilon=[0.1,~0.5,~0.9]$, 
%$\epsilon=[0.1,0.3,0.5,,0.7,0.9]$, 
versus RFFs and Baseline Kernel Ridge Regression (KRR) on a $2$-class MNIST dataset -- digits $(7,9)$. We find that $d_0=0.44$ for TRFs and $d_0=0.39$ for RFFs are numerically close, making $\lambda$ in Corollary~\ref{cor1} small. Results averaged over $5$ independent runs. }
}
\label{fig:compare_rff_ternary-MNIST}
\end{figure}

==> former_file.tex <==
Let us define 
\begin{align*}
    \Sigma &= \sigma({\bf WX})
\end{align*}
where ${\bf X}=[{\bf x}_1, \cdots, {\bf x}_n] \in \mathbb{R}^{p \times n}$ ${\bf W} \in \mathbb{R}^{m \times p}$ has i.i.d entries and $\sigma$ is applied entrywise. We consider the gram matrix
\begin{align*}
    G = \frac1m {\bm \Sigma}^{\sf T}{\bm \Sigma}
\end{align*}
whose entries are given by \\
\[
G_{ij} = \frac1m \sum_{k=1}^m \sigma({\bf w}_k^{\sf T}{\bf x}_i)\sigma({\bf w}_k^{\sf T}{\bf x}_j)\]
We are interested in computing 
\[
\Phi({\bf x}_i,{\bf x}_j)=\mathbb{E}_{{\bf w}} \sigma({\bf w}^{\sf T}{\bf x}_i)\sigma({\bf w}^{\sf T}{\bf x}_j)
\]
under the following Assumptions.
\begin{assumption}
\begin{enumerate}
    \item The entries of ${\bf w}$ are i.i.d and distributed according to $\mathcal{N}(0,1).$
    \item The activation function is three times differentiable, with $\sup_x |\sigma'(x)|, |\sigma''(x)|, |\sigma^{(3)}(x)| \le \lambda$ for some $\lambda < \infty.$
    \item For $\xi \sim \mathcal{N}(0, 1),$ we have $\mathbb{E}[\sigma(\xi)]=b_\sigma^{(0)}$ and $\mathbb{E}[\sigma(\xi^2)]=1.$ 
\end{enumerate}
\end{assumption}
%For $\xi \sim \mathcal{N}(0, 1),$ we define the following constants associated to $\sigma(x)$: \\
%$a_\sigma^{(0)} \triangleq \mathbb{E}[\sigma(\xi)^2],$
%$a_\sigma \triangleq \mathbb{E}[\sigma'(\xi)^2],$
%$b_\sigma \triangleq \mathbb{E}[\sigma'(\xi)], b_\sigma^{(2)} \triangleq \mathbb{E}[\sigma''(\xi)], b_\sigma^{(3)} \triangleq \mathbb{E}[\sigma^{(3)}(\xi)] , b_\sigma^{(4)} \triangleq \mathbb{E}[\sigma^{(4)}(\xi)], b_\sigma^{(5)} \triangleq \mathbb{E}[\sigma^{(5)}(\xi)], b_\sigma^{(6)}\triangleq \mathbb{E}[\sigma^{(6)}(\xi)].$

Observe that $({\bf w}^{\sf T}{\bf x}_i, {\bf w}^{\sf T}{\bf x}_j)$ is a bivariate Gaussian. We can perform a Gram-Schmidt orthogonalization procedure for some standard Gaussian variables $\xi_a,$ $\xi_b \in \mathcal{N}(0,1).$ We have
\begin{align*}
    {\bf w}^{\sf T}{\bf x}_i &=  u_a \xi_a \\
    {\bf w}^{\sf T}{\bf x}_j &= v_b \xi_a + u_b \xi_b
\end{align*}
with
\begin{align*}
    u_a &= \|x_i\| \\
    v_b &= \frac{{\bf x}_i^{\sf T}{\bf x}_j}{\|x_i\|} \\
    u_b &= \sqrt{\|x_j\|^2-\frac{({\bf x}_i^{\sf T}{\bf x}_j)^2}{\|x_i\|^2}}
\end{align*}
Let us denote $\zeta_a={\bf w}^{\sf T}{\bf x}_i$ and $\zeta_b={\bf w}^{\sf T}{\bf x}_j.$ We can perform a Taylor expansion of $\sigma(\zeta_a)$ (resb. $\sigma(\zeta_b)$) around $\sqrt{\tau}\xi_a$ (resp. $\sqrt{\tau}\xi_b$). We have
\begin{align*}
    \sigma(\zeta_a) &= \sigma(\sqrt{\tau}\xi_a) + \sigma'(\sqrt{\tau}\xi_a)(\zeta_a-\sqrt{\tau}\xi_a)+ \frac{1}{2}\sigma''(\xi_a)(\zeta_a-\sqrt{\tau}\xi_a)^2 +o((\zeta_a-\sqrt{\tau}\xi_a)^2) \\
        \sigma(\zeta_b) &= \sigma(\sqrt{\tau}\xi_b) + \sigma'(\sqrt{\tau}\xi_b)(\zeta_b-\sqrt{\tau}\xi_b)+ \frac{1}{2}\sigma''(\sqrt{\tau}\xi_b)(\zeta_b-\sqrt{\tau}\xi_b)^2 +o((\zeta_b-\sqrt{\tau}\xi_b)^2).
\end{align*}
We have
\begin{align*}
    \Phi({\bf x}_i,{\bf x}_j) &= \mathbb{E}[\sigma(\zeta_a)\sigma(\zeta_b)] \\
    &= \mathbb{E}[\sigma(\sqrt{\tau}\xi_a)\sigma(\sqrt{\tau}\xi_b)] + \mathbb{E}[\sigma(\sqrt{\tau}\xi_a)\sigma'(\sqrt{\tau}\xi_b)(\zeta_b-\sqrt{\tau}\xi_b)] + \frac12 \mathbb{E}[\sigma(\sqrt{\tau}\xi_a)\sigma''(\sqrt{\tau}\xi_b)(\zeta_b-\sqrt{\tau}\xi_b)^2] \\
    &+ \mathbb{E}[\sigma'(\sqrt{\tau}\xi_a)(\zeta_a-\sqrt{\tau}\xi_a)\sigma(\sqrt{\tau}\xi_b)] + \mathbb{E}[\sigma'(\sqrt{\tau}\xi_a)(\zeta_a-\sqrt{\tau}\xi_a)\sigma'(\sqrt{\tau}\xi_b)(\zeta_b-\sqrt{\tau}\xi_b)] \\ & + \frac12 \mathbb{E}[\sigma'(\xi_a)(\zeta_a-\sqrt{\tau}\xi_a)\sigma''(\xi_b)(\zeta_b-\sqrt{\tau}\xi_b)^2]
    + \frac12 \mathbb{E}[\sigma''(\xi_a)(\zeta_a-\sqrt{\tau}\xi_a)^2 \sigma(\sqrt{\tau}\xi_b)] \\&+ \frac12 \mathbb{E}[\sigma''(\sqrt{\tau}\xi_a)(\zeta_a-\sqrt{\tau}\xi_a)^2 \sigma'(\sqrt{\tau}\xi_b)(\zeta_b-\sqrt{\tau}\xi_b)] \\ &+ \frac14 \mathbb{E}[\sigma''(\sqrt{\tau}\xi_a)(\zeta_a-\sqrt{\tau}\xi_a)^2 \sigma''(\sqrt{\tau}\xi_b)(\zeta_b-\sqrt{\tau}\xi_b)^2] 
\end{align*}
Using the independence between $\xi_a, \xi_b$ along with the following
\begin{itemize}
    \item $\zeta_a-\sqrt{\tau}\xi_a = (\frac{u_a}{\sqrt{\tau}}-1)\sqrt{\tau}\xi_a$
    \item $\zeta_b-\sqrt{\tau}\xi_b = (\frac{u_b}{\sqrt{\tau}}-1)\sqrt{\tau}\xi_b + \frac{v_b}{\sqrt{\tau}} \sqrt{\tau} \xi_a$
       % \item $\mathbb{E}[\sigma(\xi)]=b_\sigma^{(0)}$
    %\item $\mathbb{E}[\xi \sigma(\xi)]= \mathbb{E}[\sigma'(\xi)]=b_\sigma$
     %\item $\mathbb{E}[\xi^2 \sigma(\xi)]= b_\sigma^{(0)}+b_\sigma^{(2)}$
    %\item $\mathbb{E}[\xi \sigma'(\xi)]= \mathbb{E}[\sigma''(\xi)]=b_\sigma^{(2)}$
     %   \item $\mathbb{E}[\xi^2 \sigma'(\xi)]= b_\sigma+b_\sigma^{(3)}$
      %  \item $\mathbb{E}[\xi \sigma''(\xi)]= b_\sigma^{(3)}$
       %         \item $\mathbb{E}[\xi^2 \sigma''(\xi)]= b_\sigma^{(2)}+b_\sigma^{(4)}$
        %\item $\mathbb{E}[\xi \sigma^{(3)}(\xi)]= b_\sigma^{(4)}$
         %       \item $\mathbb{E}[\xi^2 \sigma^{(3)}(\xi)]= b_\sigma^{(3)}+b_\sigma^{(5)}$ \\
          %      \item $\mathbb{E}[\xi^3 \sigma'(\xi)]= 3b_\sigma^{(2)}+b_\sigma^{(4)}$
           %     \item $\mathbb{E}[\xi^4 \sigma''(\xi)]= 3b_\sigma^{(2)}+6b_\sigma^{(4)}+b_\sigma^{(6)}$
\end{itemize}
we get
\begin{align}
\label{EQ1}
\Phi({\bf x}_i,{\bf x}_j) &= \left[ \left(\mathbb{E}[\sigma(\sqrt{\tau}\xi)]\right)^2 + \left(\mathbb{E}[\sigma(\sqrt{\tau}\xi)]\mathbb{E}[\sqrt{\tau}\xi\sigma'(\sqrt{\tau}\xi)]\right) \left(\frac{u_b}{\sqrt{\tau}}-1\right) + \left(\mathbb{E}[\sigma'(\sqrt{\tau}\xi)]\mathbb{E}[\sqrt{\tau}\xi\sigma(\sqrt{\tau}\xi)]\right) \frac{v_b}{\sqrt{\tau}}\right. \nonumber\\ & \left.+ \left(\mathbb{E}[\sqrt{\tau}\xi\sigma'(\sqrt{\tau}\xi)]^2\right)\left((\frac{u_a}{\sqrt{\tau}}-1)(\frac{u_b}{\sqrt{\tau}}-1)\right) + \frac{\left(\mathbb{E}[\sigma(\sqrt{\tau}\xi)]\mathbb{E}[\tau\xi^2\sigma''(\sqrt{\tau}\xi)]\right)}2\left(\left(u_b-1\right)^2\right) \right. \nonumber\\ & \left. + \frac{\left(\mathbb{E}[\sqrt{\tau}\xi\sigma'(\sqrt{\tau}\xi)]\mathbb{E}[\tau\xi^2\sigma''(\sqrt{\tau}\xi)]\right)}{2}\left(\frac{u_a}{\sqrt{\tau}} -1\right)\left(\frac{u_b}{\sqrt{\tau}} -1\right)^2 \right. \nonumber\\ & \left. + \frac{\left(\mathbb{E}[\sqrt{\tau}\xi\sigma'(\sqrt{\tau}\xi)]\mathbb{E}[\tau\xi^2\sigma''(\sqrt{\tau}\xi)]\right)}{2}\left(\frac{u_a}{\sqrt{\tau}} -1\right)^2\left(\frac{u_b}{\sqrt{\tau}} -1\right) \right. \nonumber\\ & \left.+ \frac{\left(\mathbb{E}[\tau\xi^2\sigma''(\sqrt{\tau}\xi)]^2\right)}{4}\left(\frac{u_a}{\sqrt{\tau}} -1\right)^2\left(\frac{u_b}{\sqrt{\tau}} -1\right)^2 + \left(\mathbb{E}[\sqrt{\tau}\xi\sigma(\sqrt{\tau}\xi)]\mathbb{E}[\sqrt{\tau}\xi\sigma''(\sqrt{\tau}\xi)]\right) \frac{v_b}{\sqrt{\tau}}\left(\frac{u_b}{\sqrt{\tau}} -1\right)  \right. \nonumber \\ &\left. + \frac{\left(\mathbb{E}[\sigma''(\sqrt{\tau}\xi)]\mathbb{E}[\tau\xi^2\sigma''(\sqrt{\tau}\xi)]\right)}{2}\left(\frac{v_b}{\sqrt{\tau}}\right)^2 +\left(\mathbb{E}[\sigma(\sqrt{\tau}\xi)]\mathbb{E}[\sqrt{\tau}\xi\sigma'(\sqrt{\tau}\xi)]\right) \left(\frac{u_a}{\sqrt{\tau}}-1\right)\right. \nonumber \\ &\left. + \left(\mathbb{E}[\sigma'(\sqrt{\tau}\xi)]\mathbb{E}[\xi^2\sigma'(\sqrt{\tau}\xi)]\right)\frac{v_b}{\sqrt{\tau}}\left(\frac{u_a}{\sqrt{\tau}}-1\right) + \frac{\left(\mathbb{E}[\sigma''(\sqrt{\tau}\xi)]\mathbb{E}[\tau \sqrt{\tau}\xi^3\sigma'(\sqrt{\tau}\xi)]\right)}{2}\left(\frac{v_b}{\sqrt{\tau}}\right)^2\left(\frac{u_a}{\sqrt{\tau}}-1\right) \right. \nonumber \\ &\left. +\frac{\left(\mathbb{E}[\sigma'(\sqrt{\tau}\xi)]\mathbb{E}[\tau\xi^2\sigma'(\sqrt{\tau}\xi)]\right)}{2}\frac{v_b}{\sqrt{\tau}}\left(\frac{u_a}{\sqrt{\tau}}-1\right)\left(\frac{u_b}{\sqrt{\tau}}-1\right) + \frac{\left(\mathbb{E}[\sigma(\sqrt{\tau}\xi)]\mathbb{E}[\tau\xi^2\sigma''(\sqrt{\tau}\xi)]\right)}{2}\left(\frac{u_a}{\sqrt{\tau}}-1\right)^2 \right. \nonumber \\ & \left.  + \frac{\left(\mathbb{E}[\sigma'(\sqrt{\tau}\xi)]\mathbb{E}[\tau \sqrt{\tau}\xi^3\sigma''(\sqrt{\tau}\xi)]\right)}{2}\frac{v_b}{\sqrt{\tau}}\left(\frac{u_a}{\sqrt{\tau}}-1\right)^2 \right. \nonumber \\ & \left. + \frac{\left(\mathbb{E}[\sigma''(\sqrt{\tau}\xi)]\mathbb{E}[\tau^2\xi^4\sigma''(\sqrt{\tau}\xi)]\right)}{4}\left(\frac{v_b}{\sqrt{\tau}}\right)^2\left(\frac{u_a}{\sqrt{\tau}}-1\right)^2  \right. \nonumber \\ & \left. +\frac{\left(\mathbb{E}[\sqrt{\tau}\xi \sigma''(\sqrt{\tau}\xi)]\mathbb{E}[\tau \sqrt{\tau}\xi^3\sigma''(\sqrt{\tau}\xi)]\right)}{2}\frac{v_b}{\sqrt{\tau}}\left(\frac{u_b}{\sqrt{\tau}}-1\right)\left(\frac{u_a}{\sqrt{\tau}}-1\right)^2\right]
\end{align}
Assuming $|{\bf x}_i^{\sf T}{\bf x}_j| \le \epsilon$ for a sufficiently small $\epsilon,$ we have 
\begin{align*}
\frac{u_a}{\sqrt{\tau}} - 1 &= \frac{\|x_i\|}{\sqrt{\tau}} -1\\
   \frac{u_b}{\sqrt{\tau}} - 1 = \frac{1}{\sqrt{\tau}}\sqrt{\|x_j\|^2-\frac{({\bf x}_i^{\sf T}{\bf x}_j)^2}{\|x_i\|^2}} -1 &= \left(\frac{\|x_j\|}{\sqrt{\tau}}-1\right) -\frac{1}{2\sqrt{\tau}\|x_j\|}\frac{({\bf x}_i^{\sf T}{\bf x}_j)^2}{\|x_i\|^2} \\
    \left(\frac{u_b}{\sqrt{\tau}}-1\right)^2 = \left(\frac{1}{\sqrt{\tau}} \sqrt{\|x_j\|^2-\frac{({\bf x}_i^{\sf T}{\bf x}_j)^2}{\|x_i\|^2\|x_j\|^2}} -1\right)^2 &= \left(\frac{\|x_j\|}{\sqrt{\tau}}-1\right)^2 -\frac{\frac{\|x_j\|}{\sqrt{\tau}}-1}{\|x_j\|}\frac{({\bf x}_i^{\sf T}{\bf x}_j)^2}{\|x_i\|^2} 
\end{align*}
%we obtain
%\begin{align}
%\label{Phi}
%    \Phi({\bf x}_i,{\bf x}_j) &=\left[ (b_\sigma^{(0)})^2 + b_\sigma^{(0)} b_\sigma^{(2)} \left(\left(\|x_a\| -1\right) + \left(\|x_b\| -1\right)\right) + c_{\sigma}^2\left(\left(\|x_a\| -1\right)\left(\|x_b\| -1\right)\right) \right. \nonumber\\ &\left.+ \frac{b_\sigma^{(0)}}2(b_\sigma^{(2)}+b_\sigma^{(4)})\left(\left(\|x_a\| -1\right)^2 + \left(\|x_b\| -1\right)^2\right) + \frac{\left(b_\sigma^{(2)}+b_\sigma^{(4)}\right)^2}{4}\left(\|x_a\| -1\right)^2\left(\|x_b\| -1\right)^2  \right. \nonumber \\ & \left. + \frac{b_\sigma^{(2)}}{2}\left(b_\sigma^{(2)}+b_\sigma^{(4)}\right)\left(\left(\|x_a\| -1\right)\left(\|x_b\| -1\right)\right) \left(\left(\|x_a\| -1\right)+\left(\|x_b\| -1\right)\right)\right]\nonumber \\ &+ \left[b_\sigma^2 + b_\sigma b_\sigma^{(3)} \left(\|x_b\| -1\right) + b_\sigma\left(b_\sigma+b_\sigma^{(3)}\right) \left(\|x_b\| -1\right) +b_\sigma^{(3)}\left(b_\sigma + b_\sigma^{(3)} \right)\left(\|x_a\| -1\right)\left(\|x_b\| -1\right) \right. \nonumber \\ & \left.+ \frac{b_\sigma}{2}\left( 3b_\sigma^{(3)}+ b_\sigma^{(5)}\right)\left(\|x_a\| -1\right)^2 + \frac{b_\sigma^{(3)}}{2}\left( 3b_\sigma^{(3)}+ b_\sigma^{(5)}\right)\left(\|x_a\| -1\right)^2\left(\|x_b\| -1\right) \right] \frac{{\bf x}_a^{\sf T}{\bf x}_b}{\|x_a\|} \nonumber\\ &-  \left[\frac{b_\sigma^{(0)} b_\sigma^{(2)}}{2} \frac{1}{\|{\bf x}_b\|} -  \frac{b_\sigma^{(2)}}2\left(b_\sigma^{(0)}+b_\sigma^{(2)}\right) + \frac{b_\sigma^{(0)}}2\left(b_\sigma^{(2)}+b_\sigma^{(4)}\right) \frac{\|x_b\|-1}{\|x_b\|} + \frac{(b_\sigma^{(2)})^2}2\frac{\|x_a\|-1}{\|x_b\|} \nonumber \right. \\ &\left. + \frac{b_\sigma^{(2)}}2\left(b_\sigma^{(2)}+b_\sigma^{(4)}\right) \frac{\left(\|x_a\|-1\right)\left(\|x_b\|-1\right)}{\|x_b\|} -  \frac{b_\sigma^{(2)}}2\left(3b_\sigma^{(2)}+b_\sigma^{(4)}\right) \left(\|x_a\|-1\right) + \frac{b_\sigma^{(2)}}4\left(b_\sigma^{(2)}+b_\sigma^{(4)}\right) \frac{\left(\|x_a\|-1\right)^2}{\|x_b\|} \nonumber \right. \\ &\left.  + \frac{\left(b_\sigma^{(2)}+b_\sigma^{(4)}\right)^2}{4} \frac{\left(\|x_a\|-1\right)^2\left(\|x_b\|-1\right)}{\|x_b||} - \frac{b_\sigma^{(2)} \left(3b_\sigma^{(2)} + 6b_\sigma^{(4)} +b_\sigma^{(6)} \right)}{4}\left(\|x_a\|-1\right)^2\right] \frac{({\bf x}_a^{\sf T}{\bf x}_b)^2}{\|x_a\|^2} + o(\xi^2)
%\end{align}
\section{Conjugate Kernel under GMM}
\label{sec2}
Let ${\bf x}_1,\cdots,{\bf x}_n$ be $n$ independent vectors belonging to one of $K$ distributional classes $\mathcal{C}_1, \cdots, \mathcal{C}_K.$ Class $a$ has cardinality and we assume that ${\bf x}_i$ follows a Gaussian Mixture Model (GMM) i.e., for ${\bf x}_i \in \mathcal{C}_a,$
\begin{align*}
    {\bf x}_i &= \frac{{\bm \mu}_a}{\sqrt{p}} + {\bm \omega}_i
\end{align*}
with ${\bm \omega}_i \sim \mathcal{N}({\bf 0}_p,{\bf C}_a/p)$ for some mean ${\bm \mu}_a \in \mathbb{R}^p$ and covariance ${\bf C}_a \in \mathbb{R}^{p\timesp}$ associated to $\mathcal{C}_a.$ 

We will work under the following assumptions
\begin{assumption}[Growth rate assumptions]
\label{as1}
As $n \to \infty,$
\begin{enumerate}
    \item $p/n \to c \in (0, \infty)$
    \item For each $a\in \{1,\cdots,K\}, n_a/n \to c_a \in (0, \infty)$
    \item $\|{\bm \mu}_a\|=O(1)$
    \item Letting ${\bf C}^{\circ}= \sum_{a=1}^K \frac{n_a}{n} {\bf C}_a$ and for each $a \in \{1,\cdots,K\},$ ${\bf C}_a^{\circ}={\bf C}_a-{\bf C}^{\circ}.$ Then $\|{\bf C}_a\|=O(1)$ and $tr({\bf C}_a^{\circ})=O(\sqrt{p}).$
    \item $\tau \triangleq tr({\bf C}^{\circ})/p$ converges in $(0, \infty).$
\end{enumerate}
\end{assumption}
Under Assumption~\ref{as1}, we have
\begin{align*}
    {\bf x}_i^{\sf T}{\bf x}_j &= \underbrace{{\bm \omega}_i^{\sf T}{\bm \omega}_j}_{O(p^{-\frac12})} + \underbrace{{\bm \mu}_a^{\sf T}{\bm \mu}_b/p+{\bm \mu}_a^{\sf T}{\bf w}_j/\sqrt{p}+{\bm \mu}_b^{\sf T}{\bf w}_i/\sqrt{p}}_{O(p^{-1})}
\end{align*}
and 
\begin{align*}
    \|{\bf x}_i\|^2 &= \underbrace{\tau}_{O(1)}+ \underbrace{tr({\bf C}_a^{\circ})/p+\Phi_i}_{O(p^{-\frac12})} + \underbrace{\|{\bm \mu}_a^2\|/p + 2{\bm \mu}_a^{\sf T}{\bm \omega}_i/\sqrt{p}}_{O(p^{-1})}
\end{align*}

%From Equation~\eqref{Phi}, $\Phi(a,b)$ is a smooth function of $\|{\bf x}_i\|, \|{\bf x}_j\|, {\bf x}_i^{\sf T}{\bf x}_j.$ So we can perform a Taylor approximation of $\Phi(i,j)$ by performing a Taylor expansion of $\|{\bf x}_i\|$ around $\sqrt{\tau}$ and ${\bf x}_i^{\sf T}{\bf x}_j$ around $0.$

We thus have
\begin{align*}
 %   \frac{{\bf x}_i^{\sf T}{\bf x}_j}{\|{\bf x}_i\|} &= \frac{1}{\sqrt{\tau}} \left(\underbrace{{\bm \omega}_i^{\sf T}{\bm \omega}_j}_{O(p^{-\frac12})} - \underbrace{\frac{{\bm \omega}_i^{\sf T}{\bm \omega}_j}{2\tau}\left(\frac{tr({\bf C}_a^{\circ})}{p}+\Phi_i\right)}_{O(p^{-1}} +\underbrace{\left(\frac{{\bm \mu}_a^{\sf T}{\bm \mu}_b}{p}+\frac{{\bm \mu}_a^{\sf T}{\bf w}_j}{\sqrt{p}}+\frac{{\bm \mu}_b^{\sf T}{\bf w}_i}\sqrt{p}\right)}_{O(p^{-1})} \right)+ O(p^{-\frac32}) \\
     \frac{v_b}{\sqrt{\tau}} &=\frac{{\bf x}_i^{\sf T}{\bf x}_j}{\sqrt{\tau}\|{\bf x}_i\|} = \frac{1}{\tau} \left(\underbrace{{\bm \omega}_i^{\sf T}{\bm \omega}_j}_{O(p^{-\frac12})} +\underbrace{\left(\frac{{\bm \mu}_a^{\sf T}{\bm \mu}_b}{p}+\frac{{\bm \mu}_a^{\sf T}{\bf w}_j}{\sqrt{p}}+\frac{{\bm \mu}_b^{\sf T}{\bf w}_i}\sqrt{p}\right)}_{O(p^{-1})} \right)+ O(p^{-\frac32}) \\
        \frac{\|{\bf x}_i\|}{\sqrt{\tau}}-1 &= \underbrace{\frac{1}{2\tau}\left(\frac{tr({\bf C}_a^{\circ})}{p}+\Phi_i\right)}_{O(p^{-\frac12})} + \underbrace{\frac{1}{2\tau}\left(\frac{{\|\bm \mu_a\|}^2}{p} + 2{\bm \mu}_a^{\sf T}\frac{{\bm \omega}_i}{\sqrt{p}}\right)}_{O(p^{-1})} + O(p^{-\frac32})
        \end{align*}
        \begin{align*}
                        %\left(\|{\bf x}_i\|-1\right)^2 &=
               % \left(\sqrt{\tau}-1\right)^2 \left[ 1 + \underbrace{\frac{\left(\frac{tr({\bf C}_a^{\circ})}{p}+\Phi_i\right)}{\sqrt{\tau}(\sqrt{\tau}-1)}}_{O(p^{-\frac12})} +   \underbrace{\frac{\left(\frac{{\|\bm \mu_a\|}^2}{p} + 2{\bm \mu}_a^{\sf T}\frac{{\bm \omega}_i}{\sqrt{p}}\right)}{\sqrt{\tau}(\sqrt{\tau}-1)}}_{O(p^{-1})}+
                %\underbrace{\frac{\left(\frac{tr({\bf C}_a^{\circ})}{p}+\Phi_i\right)^2}{4\tau(\sqrt{\tau}-1)^2}}_{O(p^{-1})}\right] + o(p^{-\frac32}) \\
                %\left(\|{\bf x}_i\|-1\right)^2\left(\|{\bf x}_j\|-1\right) &= \left(\sqrt{\tau}-1\right)^3
               % \left[
                %1 + \underbrace{\frac{\left(\frac{tr({\bf C}_a^{\circ})}{p}+\Phi_i\right)+\left(\frac{tr({\bf C}_b^{\circ})}{p}+\Phi_j\right)}{\sqrt{\tau}(\sqrt{\tau}-1)}}_{O(p^{-\frac12})} \right. \\ &\left. + \underbrace{\frac{\left(\frac{{\|\bm \mu_a\|}^2}{p} + 2{\bm \mu}_a^{\sf T}\frac{{\bm \omega}_i}{\sqrt{p}}\right)+\left(\frac{{\|\bm \mu_b\|}^2}{p} + 2{\bm \mu}_b^{\sf T}\frac{{\bm \omega}_j}{\sqrt{p}}\right)}{\sqrt{\tau}(\sqrt{\tau}-1)}}_{O(p^{-1})} \right.\\ &\left. + \underbrace{\frac{\left(\frac{tr({\bf C}_a^{\circ})}{p}+\Phi_i\right)^2}{4\tau(\sqrt{\tau}-1)^2}}_{O(p^{-1})} + \underbrace{\frac{\left(\frac{tr({\bf C}_a^{\circ})}{p}+\Phi_i\right)\left(\frac{tr({\bf C}_b^{\circ})}{p}+\Phi_j\right)}{2\tau(\sqrt{\tau}-1)^2}}_{O(p^{-1})}
%\right]+ O(p^{-\frac32})
\end{align*}

\begin{align*}
\left(\frac{\|{\bf x}_i\|}{\sqrt{\tau}}-1\right)\left(\frac{\|{\bf x}_j\|}{\sqrt{\tau}}-1\right) &= \underbrace{\frac{\left(\frac{tr({\bf C}_a^{\circ})}{p}+\Phi_i\right)\left(\frac{tr({\bf C}_b^{\circ})}{p}+\Phi_j\right)}{4\tau^2}}_{O(p^{-\frac12})} + O(p^{-\frac32}) \\
\left(\frac{v_b}{\sqrt{\tau}}\right)^2 &= \frac{1}{\tau^2} ({\bm \omega}_i^{\sf T}{\bm \omega}_j)^2 + O(p^{-\frac32}) \\
\frac{1}{2\sqrt{\tau}\|x_j\|}\frac{({\bf x}_i^{\sf T}{\bf x}_j)^2}{\|x_i\|^2} & = \frac{1}{2\tau^2} ({\bm \omega}_i^{\sf T}{\bm \omega}_j)^2 + O(p^{-\frac32})
%\left(\sqrt{\tau}-1\right)^2
%                \left[
%                1 + \underbrace{\frac{\left(\frac{tr({\bf C}_a^{\circ})}{p}+\Phi_i\right)+\left(\frac{tr({\bf C}_b^{\circ})}{p}+\Phi_j\right)}{2\sqrt{\tau}(\sqrt{\tau}-1)}}_{O(p^{-\frac12})} \right. \\ & \left. \underbrace{\frac{\left(\frac{{\|\bm \mu_a\|}^2}{p} + 2{\bm \mu}_a^{\sf T}\frac{{\bm \omega}_i}{\sqrt{p}}\right)+\left(\frac{{\|\bm \mu_b\|}^2}{p} + 2{\bm \mu}_b^{\sf T}\frac{{\bm \omega}_j}{\sqrt{p}}\right)}{2\sqrt{\tau}(\sqrt{\tau}-1)}}_{O(p^{-1})}  
%                \right]+ O(p^{-\frac32})
%\\
%    \left(\|{\bf x}_i\|-1\right)^2\left(\|{\bf x}_j\|-1\right)^2 &=\left(\sqrt{\tau}-1\right)^4
%                \left[
%                1 + \underbrace{\frac{\left(\frac{tr({\bf C}_a^{\circ})}{p}+\Phi_i\right)+\left(\frac{tr({\bf C}_b^{\circ})}{p}+\Phi_j\right)}{\sqrt{\tau}(\sqrt{\tau}-1)}}_{O(p^{-\frac12})} \right. \\ & \left. \underbrace{\frac{\left(\frac{{\|\bm \mu_a\|}^2}{p} + 2{\bm \mu}_a^{\sf T}\frac{{\bm \omega}_i}{\sqrt{p}}\right)+\left(\frac{{\|\bm \mu_b\|}^2}{p} + 2{\bm \mu}_b^{\sf T}\frac{{\bm \omega}_j}{\sqrt{p}}\right)}{\sqrt{\tau}(\sqrt{\tau}-1)}}_{O(p^{-1})}  \right. \\
%                                &\left.+ \underbrace{\frac{\left(\frac{tr({\bf C}_a^{\circ})}{p}+\Phi_i\right)^2+\left(\frac{tr({\bf C}_b^{\circ})}{p}+\Phi_j\right)^2}{4\tau(\sqrt{\tau}-1)^2}}_{O(p^{-1})} + \underbrace{\frac{\left(\frac{tr({\bf C}_a^{\circ})}{p}+\Phi_i\right)\left(\frac{tr({\bf C}_b^{\circ})}{p}+\Phi_j\right)}{\tau(\sqrt{\tau}-1)^2}}_{O(p^{-1})}
%                \right] + O(p^{-\frac32})
\end{align*}

%Putting all this together and denoting ${\bf t}=\left\{\frac{tr ({\bf C}_a^{\circ})}{\sqrt{p}}\right\}_{a=1}^K$, we get
%\begin{align*}
%    \Phi({\bf x}_i,{\bf x}_j) &= (b_\sigma^{(0)})^2 +2b_\sigma^{(0)} b_\sigma^{(2)}\left(\sqrt{\tau}-1\right)+\left((b_\sigma^{(2)})^2+b_\sigma^{(0)}\left(b_\sigma^{(2)}+b_\sigma^{(4)}\right)\right)\left(\sqrt{\tau}-1\right)^2 \\ &+\left(\frac{5b_\sigma^{(2)}^2+6b_\sigma^{(2)} b_\sigma^{(4)} +b_\sigma^{(4)}^2}{4}\right)\left(\sqrt{\tau}-1\right)^4\\ &+ \left(\frac{b_\sigma^{(0)} b_\sigma^{(2)}}{2\tau}+\frac{b_\sigma^{(2)}^2(\sqrt{\tau}-1)}{\sqrt{\tau}}+\frac{b_\sigma^{(0)} (b_\sigma^{(2)}+b_\sigma^{(4)})(\sqrt{\tau}-1)}{2\sqrt{\tau}}+\frac{(b_\sigma^{(2)}+b_\sigma^{(4)})^2(\sqrt{\tau}-1)^2}{4\sqrt{\tau}} \right. \\ &\left. +\frac{5b_\sigma^{(2)}(b_\sigma^{(2)}+b_\sigma^{(4)})(\sqrt{\tau}-1)^3}{4\sqrt{\tau}}\right) \\ &\times
%    \left[\left(\frac{t_a}{\sqrt{p}}+\Phi_i+\frac{t_b}{\sqrt{p}}+\Phi_j\right)+\left(\frac{{\|\bm \mu_a\|}^2}{p} + 2{\bm \mu}_a^{\sf T}\frac{{\bm \omega}_i}{\sqrt{p}}+\frac{{\|\bm \mu_b\|}^2}{p} + 2{\bm \mu}_b^{\sf T}\frac{{\bm \omega}_j}{\sqrt{p}}\right)\right]\\
    %&+\left(\frac{b_\sigma^{(0)} b_\sigma^{(2)}}{2\tau}+\frac{b_\sigma^{(2)}^2(\sqrt{\tau}-1)}{\sqrt{\tau}}+\frac{b_\sigma^{(0)} (b_\sigma^{(2)}+b_\sigma^{(4)})(\sqrt{\tau}-1)}{2\sqrt{\tau}}+\frac{5b_\sigma^{(2)}(b_\sigma^{(2)}+b_\sigma^{(4)})(\sqrt{\tau}-1)^3}{4\sqrt{\tau}} \right. \\ &\left. +\frac{(b_\sigma^{(2)}+b_\sigma^{(4)})^2(\sqrt{\tau}-1)^2}{4\sqrt{\tau}}\right\right)\left(\frac{{\|\bm \mu_a\|}^2}{p} + 2{\bm \mu}_a^{\sf T}\frac{{\bm \omega}_i}{\sqrt{p}}+\frac{{\|\bm \mu_b\|}^2}{p} + 2{\bm \mu}_b^{\sf T}\frac{{\bm \omega}_j}{\sqrt{p}}\right) \\
 %   &+ \left(\frac{b_\sigma^{(2)}(b_\sigma^{(2)}+b_\sigma^{(4)})(\sqrt{\tau}-1)^2}{4\tau}\right)\left[\left(\frac{t_a}{\sqrt{p}}+\Phi_i\right)\left(\frac{t_b}{\sqrt{p}}+\Phi_j\right)\right] \\
 %   &+ \left(\frac{b_\sigma^{(0)}(b_\sigma^{(2)}+b_\sigma^{(4)})}{8\tau}+\frac{(b_\sigma^{(2)}+b_\sigma^{(4)})^2(\sqrt{\tau}-1)^2}{16\tau}+\frac{b_\sigma^{(2)}(b_\sigma^{(2)}+b_\sigma^{(4)})(\sqrt{\tau}-1)^2}{8\tau}\right) \\ &\left[\left(\frac{t_a}{\sqrt{p}}+\Phi_i\right)^2+\left(\frac{t_b}{\sqrt{p}}+\Phi_j\right)^2\right] \\
  %  &+\frac{1}{\sqrt{\tau}}\left(b_\sigma^2+\left(\sqrt{\tau}-1\right) \left(b_\sigma b_\sigma^{(3)}+(\sqrt{\tau}-1) \left(b_\sigma (b_\sigma^{(3)}+b_\sigma)+b_\sigma^{(3)}(b_\sigma+b_\sigma^{(3)})+\frac{b_\sigma}2(3b_\sigma^{(3)}+b_\sigma^{(5)})\right. \\ &\left. +\frac{b_\sigma^{(3)}}2(3b_\sigma^{(3)}+b_\sigma^{(5)})\right)\right)\right) \\ &\times
%\left(\frac{{\bm \mu}_a^{\sf T}{\bm \mu}_b}{p}+\frac{{\bm \mu}_a^{\sf T}{\bm \omega}_j}{\sqrt{p}}+\frac{{\bm \mu}_b^{\sf T}{\bm \omega}_i}{\sqrt{p}} +{\bm \omega}_i^{\sf T}{\bm \omega}_j\right) \\
    %\left(\frac{b_\sigma^{(0)}(b_\sigma^{(2)}+b_\sigma^{(4)})}{8\tau}+\frac{b_\sigma^{(0)}(b_\sigma^{(2)}+b_\sigma^{(4)})(\sqrt{\tau}-1)^2}{8\tau}+\frac{(b_\sigma^{(2)}+b_\sigma^{(4)})^2(\sqrt{\tau}-1)}{16\tau}\right)\left(\frac{t_b}{\sqrt{p}}+\Phi_j\right)^2 \\
      %                  &+\left(\frac{b_\sigma^{(0)} b_\sigma^{(2)}}{2\sqrt{\tau}}-\frac{b_\sigma^{(2)}(b_\sigma^{(0)}+b_\sigma^{(2)})}{2}+ \frac{(\sqrt{\tau}-1)}{2\sqrt{\tau}}\left(b_\sigma^{(0)} b_\sigma^{(2)} +b_\sigma^{(0)} b_\sigma^{(4)} -2b_\sigma^{(2)}^2-b_\sigma^{(2)} b_\sigma^{(4)}\right) \right. \\ &\left. + \frac{(\sqrt{\tau}-1)^2}{4\sqrt{\tau}}\left(4(b_\sigma^{(2)})^2+5b_\sigma^{(2)} b_\sigma^{(4)}+b_\sigma^{(4)}^2\right)-\frac{(\sqrt{\tau}-1)^2}{4}\left(3(b_\sigma^{(2)})^2+6b_\sigma^{(2)} b_\sigma^{(4)}+b_\sigma^{(2)} b_\sigma^{(6)}\right)\right)\left({\bm \omega}_i^{\sf T}{\bm \omega}_j\right)^2\\
    %&-\frac{1}{\tau}\left(\frac{b_\sigma^2}{2 \sqrt{\tau}}+\left(2b_\sigma b_\sigma^{(3)}+b_\sigma^{(3)}^2\right)\frac{ (\sqrt{\tau}-1)}{2\sqrt{\tau}}\right.\\ &\left. -\left[\frac{b_\sigma^{(3)}}{2}(3b_\sigma^{(3)}+b_\sigma^{(5)})+\frac{b_\sigma}{2}(3b_\sigma^{(3)}+b_\sigma^{(5)})+b_\sigma^{(3)}(b_\sigma+b_\sigma^{(3)})\right]\frac{\left(\tau-1\right)}{2 \sqrt{\tau}}\right) \left({\bm \omega}_i^{\sf T}{\bm \omega}_j\left(\frac{t_a}{\sqrt{p}}+\Phi_i\right)\right)\\
    %    &+\frac{1}{\tau}\left(\frac{\left(2b_\sigma b_\sigma^{(3)}+b_\sigma^2\right)}{2\sqrt{\tau}}+\left(4b_\sigma^{(3)}^2+b_\sigma b_\sigma^{(3)}+b_\sigma^{(3)} b_\sigma^{(5)}\right)\left(\sqrt{\tau}-1\right)\right)\left({\bm \omega}_i^{\sf T}{\bm \omega}_j\left(\frac{t_b}{\sqrt{p}}+\Phi_j\right)\right) \\
               % &+\left(\frac{b_\sigma^{(3)}(b_\sigma+b_\sigma^{(3)})(\sqrt{\tau}-1)}{\sqrt{\tau}}+\frac{b_\sigma^{(3)}(3b_\sigma^{(3)}+b_\sigma^{(5)})(\sqrt{\tau}-1)^2}{\sqrt{\tau}}\right)\left({\bm \omega}_i^{\sf T}{\bm \omega}_j\left(\frac{t_a}{\sqrt{p}}+\Phi_i\right)\left(\frac{t_b}{\sqrt{p}}+\Phi_j\right)\right) \\
 %&+ O(p^{-\frac32})
%\end{align*}
All other terms in Equation~\eqref{EQ1} are vanishing asymptotically. We get
we get
\begin{align}
\label{EQ2}
\Phi({\bf x}_i,{\bf x}_j) &= \left[ \left(\mathbb{E}[\sigma(\sqrt{\tau}\xi)]\right)^2 + \left(\mathbb{E}[\sigma(\sqrt{\tau}\xi)]\mathbb{E}[\sqrt{\tau}\xi\sigma'(\sqrt{\tau}\xi)]\right) \left(\frac{u_b}{\sqrt{\tau}}-1\right) + \left(\mathbb{E}[\sigma'(\sqrt{\tau}\xi)]\mathbb{E}[\sqrt{\tau}\xi\sigma(\sqrt{\tau}\xi)]\right) \frac{v_b}{\sqrt{\tau}}+ \right. \nonumber\\ & \left.+ \left(\mathbb{E}[\sqrt{\tau}\xi\sigma'(\sqrt{\tau}\xi)]^2\right)\left((\frac{u_a}{\sqrt{\tau}}-1)(\frac{u_b}{\sqrt{\tau}}-1)\right) + \frac{\left(\mathbb{E}[\sigma''(\sqrt{\tau}\xi)]\mathbb{E}[\tau\xi^2\sigma(\sqrt{\tau}\xi)]\right)}{2}\left(\frac{v_b}{\sqrt{\tau}}\right)^2 \right. \nonumber \\ &\left. +\left(\mathbb{E}[\sigma(\sqrt{\tau}\xi)]\mathbb{E}[\sqrt{\tau}\xi\sigma'(\sqrt{\tau}\xi)]\right) \left(\frac{u_a}{\sqrt{\tau}}-1\right)\right]
\end{align}
Let us denote
\begin{align*}
{\bf P} &={\bf I}-\frac1n {\bf 11}^{\sf T} \\
    {\bm \Omega} &= [{\bm \omega}_1, \cdots, {\bm \omega}_n] \\
    {\bm \Phi} &=\left\{\|{\bm \omega}_i\|^2-\mathbb{E}[\|{\bm \omega}_i\|^2]\right\}_{i=1}^n \\
    {\bf M} &= [{\bm \mu}_1,\cdots, {\bm \mu}_K] \\
    {\bf t} &=\left\{\frac{tr ({\bf C}_a^{\circ})}{\sqrt{p}}\right\}_{a=1}^K\\
    {\bf S} &= \left\{\frac{tr {\bf C}_a{\bf C}_b}{p} \ \right\}_{a,b=1}^K \\
    {\bf J} &= [{\bf j}_1, \cdots, {\bf j}_K].
\end{align*}
After simplifications, we can write
\begin{align*}
    \|{\bf P}{\bm \Phi}{\bf P}-{\bf P}\tilde{{\bm \Phi}}{\bf P}\| \to 0
\end{align*}
as $n\to \infty$ almost surely, 
where
\begin{align}
    \tilde{{\bm \Phi}} &= d_1 {\bm \Omega}^{\sf T}{\bm \Omega} + {\bf VAV}^{\sf T} + d_0{\bf I}
    \label{EQ6}
\end{align}
\begin{align*}
    {\bf V} &= \left[\frac{{\bf J}}{\sqrt{p}}, \Phi, \frac{1}{\sqrt{p}}{\bm \Omega}^{\sf T}{\bf M}\right]\\
    {\bf A} &= \left[\begin{matrix}
    {\bf A}_{11} & d_2 {\bf t} & d_1{\bf I}_K \\
    d_2 {\bf t}^{\sf T} & d_2 & 0\\
    d_1{\bf I}_K & 0 & 0
    \end{matrix}\right]
\end{align*}
\begin{align*}
    {\bf A}_{11} &= d_1 {\bf M}^{\sf T}{\bf M} +d_2 {\bf t}^{\sf T}{\bf t} +d_3 {\bf S}
\end{align*}
and the constants $d_0, d_1, d_2, d_3$ are as follows
\begin{align*}
%d_0 &= (b_\sigma^{(0)})^2 + 2b_\sigma^{(0)} b_\sigma^{(2)} \left(\sqrt{\tau}-1\right) + \left(\frac{b_\sigma^{(0)}}{2}\left(b_\sigma^{(2)}+b_\sigma^{(4)}\right)+(b_\sigma^{(2)})^2\right)\left(\sqrt{\tau}-1\right)^2 + \left(b_\sigma^{(2)}\left(b_\sigma^{(2)}+b_\sigma^{(4)}\right)\right)\left(\sqrt{\tau}-1\right)^3 \\ &+ \left(\frac{\left(b_\sigma^{(2)}+b_\sigma^{(4)}\right)^4}{4}\right)\left(\sqrt{\tau}-1\right)^4 \\
d_0 & = \mathbb{E}[\sigma(\sqrt{\tau}\xi)^2] - \mathbb{E}[\sigma(\sqrt{\tau}\xi)]^2 - \sqrt{\tau} \mathbb{E}[\sigma'(\sqrt{\tau}\xi)]\mathbb{E}[\xi\sigma(\sqrt{\tau}\xi)] \\
%d_0 &= \frac12 \left[\mathbb{E}[\sigma(\xi)^2]+\left(\sqrt{\tau-1}\right)^2\mathbb{E}[\xi^2 \left(\sigma'(\xi)\right)^2] +\frac14\left(\sqrt{\tau-1}\right)^4\mathbb{E}[\xi^4 \left(\sigma''(\xi)\right)^2] \right. \\ &\left. + 2\left(\sqrt{\tau-1}\right)\mathbb{E}[\xi \sigma(\xi)\sigma'(\xi)] +\left(\sqrt{\tau-1}\right)^2\mathbb{E}[\xi^2 \sigma(\xi)\sigma''(\xi)]+\left(\sqrt{\tau-1}\right)^3\mathbb{E}[\xi^3 \sigma'(\xi)\sigma''(\xi)]\right] \\
%&- \left[ \mathbb{E}[\sigma(\xi)]^2 +2\mathbb{E}[\sigma(\xi)]\mathbb{E}[\xi \sigma'(\xi)]\left(\sqrt{\tau}-1\right)+\left(\mathbb{E}[\xi\sigma'(\xi)]^2+\mathbb{E}[\sigma(\xi)]\mathbb{E}[\xi^2 \sigma''(\xi)]\right)\left(\sqrt{\tau}-1\right)^2 \right. \\ &\left. +\mathbb{E}[\xi\sigma'(\xi)]\mathbb{E}[\xi^2 \sigma''(\xi)]\left(\sqrt{\tau}-1\right)^3+\frac{\mathbb{E}[\xi^2\sigma''(\xi)]}{4}\left(\sqrt{\tau}-1\right)^4 \right]\\
%    d_1 &= \frac{\mathbb{E}[\sigma'(\xi)]\mathbb{E}[\xi\sigma(\xi)]}{\tau} + \frac{\left(\sqrt{\tau}-1\right)}{\tau} \left(\mathbb{E}[\xi\sigma''(\xi)]\mathbb{E}[\xi\sigma(\xi)]+\mathbb{E}[\sigma'(\xi)]\mathbb{E}[\xi^2\sigma'(\xi)]+\frac{\mathbb{E}[\xi^3\sigma''(\xi)]\mathbb{E}[\sigma'(\xi)]}{2}\right) \\ &+ \frac{\left(\sqrt{\tau}-1\right)^2}{\tau}\left(\mathbb{E}[\xi\sigma''(\xi)]\mathbb{E}[\xi^2\sigma'(\xi)]\right) +\frac{\left(\sqrt{\tau}-1\right)^3}{\tau} \left(\mathbb{E}[\xi^3\sigma''(\xi)]\mathbb{E}[\xi\sigma''(\xi)]\right) \\
d_1& = \frac{\mathbb{E}[\sigma'(\sqrt{\tau}\xi)]\mathbb{E}[\xi\sigma(\sqrt{\tau}\xi)]}{\sqrt{\tau}} \\
%    d_2 &= \frac{1}{\tau} \left[\mathbb{E}[\xi\sigma'(\xi)]+\left(\sqrt{\tau}-1\right)\mathbb{E}[\xi^2\sigma''(\xi)]\right]^2 \\
d_2 &= \frac{\mathbb{E}[\xi\sigma'(\sqrt{\tau}\xi)]^2}{4\tau} \\
d_3 &= \frac{\mathbb{E}[\sigma''(\sqrt{\tau}\xi)]\mathbb{E}[\xi^2\sigma(\sqrt{\tau}\xi)]}{2\tau} - \frac{\mathbb{E}[\xi\sigma'(\sqrt{\tau}\xi)]\mathbb{E}[\sigma(\sqrt{\tau}\xi)]}{2\tau\sqrt{\tau}}
   % d_3 &= \left(\frac{\mathbb{E}[\sigma''(\xi)]\mathbb{E}[\xi^2\sigma(\xi)]}{2}\right)\frac{1}{\tau} - \left(\frac{\mathbb{E}[\xi\sigma'(\xi)]\mathbb{E}[\sigma(\xi)]}{2}\right) \frac{1}{\tau\sqrt{\tau}} \\ &- \left(\frac{\left(\mathbb{E}[\xi\sigma'(\xi)]\right)^2}{2}+\frac{\mathbb{E}[\sigma(\xi)]\mathbb{E}[\xi^2\sigma''(\xi)]}{2}-\frac{\mathbb{E}[\sigma''(\xi)]\mathbb{E}[\xi^3\sigma'(\xi)]}{2}\right) \frac{\left(\sqrt{\tau}-1\right)}{\tau\sqrt{\tau}} \\  &- \left(\frac{\mathbb{E}[\sigma'(\xi)]\mathbb{E}[\xi^2\sigma''(\xi)]}{2}+\frac{\mathbb{E}[\xi\sigma'(\xi)]\mathbb{E}[\xi^2\sigma''(\xi)]}{4}\right) \frac{\left(\sqrt{\tau}-1\right)^2}{\tau\sqrt{\tau}} + \left(\frac{\mathbb{E}[\sigma''(\xi)]\mathbb{E}[\xi^4\sigma''(\xi)]}{4}\right)\left(\sqrt{\tau}-1\right)^2 \\ &- \left(\frac{\left(\mathbb{E}[\xi^2\sigma''(\xi)]\right)^2}{4}\right) \frac{\left(\sqrt{\tau}-1\right)^3}{\tau\sqrt{\tau}}
\end{align*}

By applying Stein's Lemma for activation functions $\sigma$ differentiable everywhere,
we get 
\begin{align*}
    d_0 &=  \mathbb{E}[\sigma(\sqrt{\tau}\xi)^2] - \mathbb{E}[\sigma(\sqrt{\tau}\xi)]^2 - \tau \mathbb{E}[\sigma'(\sqrt{\tau}\xi)]^2 \\
    d_1 &= \mathbb{E}[\sigma'(\sqrt{\tau}\xi)]^2 \\
    d_2 &= \frac{\mathbb{E}[\sigma''(\sqrt{\tau}\xi)]^2}{4} \\
    d_3 &= \frac{\mathbb{E}[\sigma''(\sqrt{\tau}\xi)]^2}{2} = 2d_2
\end{align*}

{\RED ** Romain ** Ce serait bien de lister des cas particuliers et de mettre quelques figures. Notamment comparer aux résultats (i) qu'on connait déjà pour les fonctions "simples", dérivables, (ii) de Zhenyu pour les fonctions pas différentiables partout. }

In order to evaluate the key quantities $d_0, d_1, d_2, d_3,$ we need to evaluate for each activation function $\sigma$, for $\xi \sim N(0,1),$ the expectation of the form $\mathbb{E}[\left(\sigma^{(d)}(\sqrt{\tau}\xi)\right)^n],$ ($n=1,2; d=0,1,2$) with $\sigma^{(d)}(\xi),$ the $d$-th derivative of $\sigma(\xi)$
\subsection{Particular cases}
\begin{center}
\renewcommand{\arraystretch}{2}
\begin{tabular}{|c|c|c|c|c|c|p{5cm}|} 
 \hline
 Expectations & $\max(0,\xi)$ & $a_{+}\max(0,\xi) + a_{-}\max(0,-\xi)$ & $a_2\xi^2+a_1\xi+a_0$ & $\exp{\left(-\xi^2/2\right)}$\\
 \hline
% $\mathbb{E}\left[\sigma(\xi)\right]$  & $\frac{1}{\sqrt{2\pi}}$  & $\frac{a_{+}+a_{-}}{\sqrt{2\pi}}$ & $a_0+a_2$ & $\frac{1}{\sqrt{2}}$ \\
$\mathbb{E}\left[\sigma(\sqrt{\tau}\xi)\right]$  & $\frac{\sqrt{\tau}}{\sqrt{2\pi}}$  & $\frac{\sqrt{\tau}(a_{+}+a_{-})}{\sqrt{2\pi}}$ & $a_0+a_2\tau$ & $\frac{1}{\sqrt{\tau+1}}$ \\
  \hline
 %$\mathbb{E}\left[\sigma'(\xi) \right]$ & $\frac12$ &  $\frac{a_{+}-a_{-}}{2}$ & $a_1$ & $0$ \\ 
 $\mathbb{E}\left[\sigma'(\sqrt{\tau}\xi) \right]$ & $\frac{1}2$ &  $\frac{a_{+}-a_{-}}{2}$ & $a_1$ & $0$ \\
 \hline
% $\mathbb{E}\left[\sigma''(\xi)\right]$  & $0$ & $0$ & $2a_2$ & $-\frac{1}{2\sqrt{2}}$ \\ 
 $\mathbb{E}\left[\sigma''(\sqrt{\tau}\xi)\right]$  & $\frac{2}{\sqrt{2\pi}}$ & $\frac{2(a_{+}+a_{-})}{\sqrt{2\pi}}$ & $2a_2$ & $\frac{\tau}{(\tau+1)\sqrt{\tau+1}}-\frac{1}{\sqrt{\tau+1}}$ \\ 
  \hline
%   $\mathbb{E}\left[\xi \sigma(\xi)\right]$  & $\frac12$ & $\frac{a_{+}-a_{-}}{2}$ & $a_1$ &$0$\\
 %$\mathbb{E}\left[\xi \sigma(\sqrt{\tau}\xi)\right]$  & $\frac{\sqrt{\tau}}2$ & $\frac{\sqrt{\tau}(a_{+}-a_{-})}{2}$ & $a_1\sqrt{\tau}$ &$0$\\
 % \hline
  %$  \mathbb{E}\left[\xi \sigma'(\xi)\right]$ & $\frac{1}{\sqrt{2\pi}}$ & $\frac{a_{+}-a_{-}}{\sqrt{2\pi}}$ & $2 a_2 $& $\frac{1}{2\sqrt{2}}$\\
  %$  \mathbb{E}\left[\xi \sigma'(\sqrt{\tau}\xi)\right]$ & $\frac{1}{\sqrt{2\pi}}$ & $\frac{a_{+}-a_{-}}{\sqrt{2\pi}}$ & $2 a_2 \sqrt{\tau} $& $-\frac{\sqrt{\tau}}{(\tau+1)\sqrt{\tau+1}}$\\
  %\hline
  % \hline
  % $ \mathbb{E}\left[\xi \sigma''(\xi)\right]$ & $0$ & $0$ & $0$ & $0$\\
%    $\mathbb{E}\left[\xi^2\sigma(\xi)\right]$ & $\frac{2}{\sqrt{2\pi}}$ & $\frac{2(a_{+}-a_{-})}{\sqrt{2\pi}}$ & $3a_2+a_0$ & $\frac{1}{2\sqrt{2}}$\\
       % $\mathbb{E}\left[\xi^2\sigma(\sqrt{\tau}\xi)\right]$ & $\frac{2}{\sqrt{2\pi}}$ & $\frac{2(a_{+}-a_{-})}{\sqrt{2\pi}}$ & $3a_2+a_0$ & $\frac{1}{2\sqrt{2}}$\\
 %    \hline
 %   $\mathbb{E}\left[\xi^2\sigma'(\xi)\right]$ & $\frac12$ & $\frac{a_{+}-a_{-}}{2}$  & $a_1$ & $0$\\
 %    \hline
 %   $\mathbb{E}\left[\xi^2\sigma''(\xi)\right]$ & $0$ & $0$  & $2a_2$ &  $\frac{3}{4\sqrt{2}}$\\
 %    \hline
 %   $\mathbb{E}\left[\xi^3 \sigma'(\xi)\right]$ & $0$ & $0$ & $6a_2$ & $-\frac{3}{4\sqrt{2}}$\\
 %    \hline
 %   $\mathbb{E}\left[\xi^3\sigma''(\xi)\right]$ & $0$ & $0$ & $0$ &  0\\
 %    \hline
 %   $\mathbb{E}\left[\xi^4\sigma''(\xi)\right]$ & $0$ & $0$ & $6a_2$&  $\frac{15}{8\sqrt{2}}$\\
 %    \hline
 %   $\mathbb{E}\left[\xi^4(\sigma''(\xi))^2\right]$ & $0$ & $0$ & $12a_2^2$ & $\frac{35}{27\sqrt{3}}$\\
    
 %    \hline
   %  $\mathbb{E}\left[\sigma(\xi)^2\right]$ & $\frac12$ & $\frac{a_{+}^2+a_{-}^2}{2}$ &  $a_0^2+a_1^2+3a_2^2+2a_2a_0$ & $\frac{1}{\sqrt{3}}$ \\
    $\mathbb{E}\left[\sigma(\sqrt{\tau}\xi)^2\right]$ & $\frac{\tau}2$ & $\frac{\tau(a_{+}^2+a_{-}^2)}{2}$ &  $\begin{matrix}a_0^2+a_1^2\tau+3a_2^2\tau^2 \\ +2a_2a_0\tau \end{matrix}$ & $\frac{1}{\sqrt{2\tau+1}}$ \\
 %    \hline
 %   $\mathbb{E}\left[\xi\sigma(\xi)\sigma'(\xi)\right]$ & $\frac12$ & $\frac{a_{+}^2+a_{-}^2}{2}$ & $6a_2^2+a_1^2+2a_2a_0$ & $-\frac{1}{\sqrt{3}}$\\
 %    \hline
 %   $\mathbb{E}\left[\xi^2\sigma(\xi)\sigma''(\xi)\right]$ & $0$ & $0$ &$6a_2^2+2a_2a_0$ & $\frac{1}{3\sqrt{3}}$\\
 %    \hline
 %   $\mathbb{E}\left[\xi^3 \sigma'(\xi)\sigma''(\xi)\right]$ & $0$ & $0$ & $0$ & $-\frac{5}{9\sqrt{3}}$\\
 %    \hline
  %  $\mathbb{E}\left[\xi^2 (\sigma'(\xi))^2\right]$ & $\frac12$ & $\frac{a_{+}^2+a_{-}^2}{2}$ & $12a_2^2+a_1^2$ & $\frac{1}{3\sqrt{3}}$\\
 \hline
\end{tabular}
\end{center}

\begin{center}
\renewcommand{\arraystretch}{2}
\begin{tabular}{|c|c|c|c|c|c|c|}
 \hline
 Expectations & $\cos{t}$ & $\sin{t}$ & $|t|$ & $t$ & $sign(t)$ & $1_{t>0}$\\
 \hline
 %$\mathbb{E}\left[\sigma(\xi)\right]$  & $e^{-\frac12}$  & $0$ & $\frac{2}{\sqrt{2\pi}}$ & $0$ & $\frac12$ & $0$ \\ 
  $\mathbb{E}\left[\sigma(\sqrt{\tau}\xi)\right]$  & $e^{-\frac{\tau}2}$  & $0$ & $\frac{2\sqrt{\tau}}{\sqrt{2\pi}}$ & $0$ & $0$ & $\frac12$\\ 
  \hline
 %$\mathbb{E}\left[\sigma'(\xi) \right]$ & $0$ &  $e^{-\frac12}$ & $0$ & $0$ & $0$ &$1$ \\ 
  $\mathbb{E}\left[\sigma'(\sqrt{\tau}\xi) \right]$ & $0$ &  $\sqrt{\tau}e^{-\frac{\tau}2}$ & $0$ & $1$ & $\frac{2}{\sqrt{2\pi\tau}}$ & $\frac{1}{\sqrt{2\pi \tau}}$\\ 
  \hline
  % $\mathbb{E}\left[\sigma''(\xi)\right]$  & $-e^{-\frac12}$ & $0$ & $0$ & $0$ & $0$ & $0$\\ 
 $\mathbb{E}\left[\sigma''(\sqrt{\tau}\xi)\right]$  & $-e^{-\frac{\tau}2}$ & $0$ & $0$ & $0$ & $0$ & $0$\\ 
 % \hline
   %$\mathbb{E}\left[\xi \sigma(\xi)\right]$  & $0$ & $e^{-\frac12}$ & $0$ &$\frac{2}{\sqrt{2\pi}}$ & $1$ & $1$\\
% $\mathbb{E}\left[\xi \sigma(\sqrt{\tau}\xi)\right]$  & $0$ & $\sqrt{\tau}e^{-\frac{\tau}2}$ & $0$ &$\sqrt{\tau}$ & $2$ & $\frac{1}{\sqrt{2\pi}}$\\
 % \hline
 % $  \mathbb{E}\left[\xi \sigma'(\xi)\right]$ & $-e^{-\frac12}$ & $0$ & $\frac{2}{\sqrt{2\pi}}$& $0$ & $0$ & $0$\\
  %  $  \mathbb{E}\left[\xi \sigma'(\sqrt{\tau}\xi)\right]$ & $-\sqrt{\tau}e^{-\frac{\tau}2}$ & $0$ & $\frac{2\sqrt{\tau}}{\sqrt{2\pi}}$& $0$ & $0$ & $0$\\
   \hline
  % $ \mathbb{E}\left[\xi \sigma''(\xi)\right]$ & $0$ & $-e^{-\frac12}$ & $0$ & $0$ & $0$ & $0$\\
  %  \hline
  %      $\mathbb{E}\left[\xi^2\sigma(\xi)\right]$ & $0$ & $0$ & $0$ & $0$ & $\frac12$ & $0$\\
   % $\mathbb{E}\left[\xi^2\sigma(\sqrt{\tau}\xi)\right]$ & $(1-\tau)e^{-\frac{\tau}{2}}$ & $0$ & $0$ & $0$ & $0$ & $0$\\
%     \hline
 %   $\mathbb{E}\left[\xi^2\sigma'(\xi)\right]$ & $0$ & $0$  & $0$ & $0$ & $0$ & $1$\\
 %   $\mathbb{E}\left[\xi^2\sigma''(\xi)\right]$ & $0$ & $0$  & $0$ &  $0$ & $0$ & $0$\\
 %    \hline
 %   $\mathbb{E}\left[\xi^3 \sigma'(\xi)\right]$ & $-2e^{-\frac12}$ & $0$ & $0$ & $0$ & $0$ & $0$\\
%     \hline
%    $\mathbb{E}\left[\xi^3\sigma''(\xi)\right]$ & $0$ & $-2e^{-\frac12}$ & $0$ &  $0$ & $0$ & $0$\\
  %  $\mathbb{E}\left[\xi^4\sigma''(\xi)\right]$ & $2e^{-\frac12}$ & $0$ & $0$&  $0$ & $0$ & $0$\\
  %  $\mathbb{E}\left[\xi^4(\sigma''(\xi))^2\right]$ & $\frac12 \left(3-5e^{-2}\right)$ & $\frac12 \left(3+5e^{-2}\right)$ & $0$ & $0$ & $0$ & $0$\\
    
  %   \hline
  %       $\mathbb{E}\left[\sigma(\sqrt{\tau}\xi)^2\right]$ & $\frac{1+e^{-2}}{2}$ & $\frac12 \left(1-e^{-2}\right)$ &  $1$ & $1$ & $\frac12$ & $1$\\
    $\mathbb{E}\left[\sigma(\sqrt{\tau}\xi)^2\right]$ & $\frac{1+e^{-2\tau}}{2}$ & $\frac{1-e^{-2\tau}}{2}$ &  $\sqrt{\tau}$ & $\sqrt{\tau}$ & $1$ & $\frac12$\\
 %    \hline
 %   $\mathbb{E}\left[\xi\sigma(\xi)\sigma'(\xi)\right]$ & $-e^{-2}$ & $e^{-2}$ & $1$ & $0$ & $0$ & $1$\\
 %    \hline
%    $\mathbb{E}\left[\xi^2\sigma(\xi)\sigma''(\xi)\right]$ & $-\left(\frac{1-3e^{-2}}{2}\right)$ & $-\left(\frac{1+3e^{-2}}{2}\right)$ &$0$ & $0$ & $0$ & $0$\\
%     \hline
%    $\mathbb{E}\left[\xi^3 \sigma'(\xi)\sigma''(\xi)\right]$ & $-e^{-2}$ & $e^{-2}$ & $0$ & $0$ & $0$ & $0$\\
   % $\mathbb{E}\left[\xi^2 (\sigma'(\xi))^2\right]$ & $\frac{1+3e^{-2}}{2}$ & $\frac{1-3e^{-2}}{2}$ & $1$ & $0$ & $0$ & $1$\\
 \hline
\end{tabular}
\end{center}


%\setlength{\tabcolsep}{30pt}



%\begin{figure}[h!]
%  \centering
%  \begin{tikzpicture}[font=\footnotesize]
%    \renewcommand{\axisdefaulttryminticks}{4} 
%    \tikzstyle{every major grid}+=[style=densely dashed]       
 %   \tikzstyle{every axis y label}+=[yshift=-10pt] 
%    \tikzstyle{every axis x label}+=[yshift=5pt]
 %   \tikzstyle{every axis legend}+=[cells={anchor=west},fill=white,
 %       at={(0.98,0.98)}, anchor=north east, font=\scriptsize ]
 %   \begin{axis}[
      %ybar,
 %     height=\textwidth,
 %     width=\textwidth,
 %     xmin=-1.5,
 %     ymin=0,
 %     xmax=8,
 %     ymax=1.2,
      %xtick={0,1,2,3,4},
      %ytick={0,0.2,0.4,0.6,0.8},
 %     yticklabels={},
 %     bar width=3pt,
 %     grid=none,
 %     ymajorgrids=false,
 %     scaled ticks=false,
      %axis x line = middle,
    	  %axis y line = middle,
      %xticklabels={}
      %scaled ticks=true,
      %scale ticks above={4},
      %xlabel={Eigenvalues},
      %ylabel={Density}
      %]
      %art
  %    \addplot[area %legend,ybar,mark=none,color=black,fill=blue] coordinates{
%(-1.295509, 0.000000)(-1.165958, 0.000000)(-1.036407, 0.000000)(-0.906856, 0.000000)(-0.777305, 0.000000)(-0.647754, 0.000000)(-0.518204, 0.000000)(-0.388653, 0.000000)(-0.259102, 0.000000)(-0.129551, 0.000000)(0.000000, 0.508819)(0.129551, 0.970525)(0.259102, 0.650158)(0.388653, 0.478667)(0.518204, 0.365596)(0.647754, 0.288331)(0.777305, 0.226142)(0.906856, 0.169606)(1.036407, 0.124378)(1.165958, 0.071612)(1.295509, 0.003769)(1.425060, 0.000000)(1.554611, 0.000000)(1.684162, 0.000000)(1.813712, 0.000000)(1.943263, 0.000000)(2.072814, 0.000000)(2.202365, 0.000000)(2.331916, 0.000000)(2.461467, 0.000000)(2.591018, 0.000000)(2.720569, 0.000000)(2.850120, 0.000000)(2.979671, 0.000000)(3.109221, 0.000000)(3.238772, 0.000000)(3.368323, 0.000000)(3.497874, 0.000000)(3.627425, 0.000000)(3.756976, 0.000000)(3.886527, 0.000000)(4.016078, 0.000000)(4.145629, 0.000000)(4.275179, 0.000000)(4.404730, 0.000000)(4.534281, 0.000000)(4.663832, 0.000000)(4.793383, 0.000000)(4.922934, 0.000000)(5.052485, 0.000000)(5.182036, 0.000000)(5.311587, 0.000000)(5.441137, 0.000000)(5.570688, 0.000000)(5.700239, 0.000000)(5.829790, 0.000000)(5.959341, 0.000000)(6.088892, 0.000000)(6.218443, 0.000000)(6.347994, 0.000000)(6.477545, 0.02)(6.607095, 0.000000)(6.736646, 0.000000)(6.866197, 0.000000)(6.995748, 0.000000)(7.125299, 0.000000)(7.254850, 0.000000)(7.384401, 0.000000)(7.513952, 0.000000)(7.643503, 0.000000)(7.773053, 0.000000)};
%\addplot[area legend,ybar,mark=none,color=black,fill=red] coordinates{
%(-1.295509, 0.000000)(-1.165958, 0.000000)(-1.036407, 0.000000)(-0.906856, 0.000000)(-0.777305, 0.000000)(-0.647754, 0.000000)(-0.518204, 0.000000)(-0.388653, 0.000000)(-0.259102, 0.000000)(-0.129551, 0.001885)(0.000000, 0.246871)(0.129551, 1.044021)(0.259102, 0.733076)(0.388653, 0.559701)(0.518204, 0.435323)(0.647754, 0.342982)(0.777305, 0.258179)(0.906856, 0.175260)(1.036407, 0.060304)(1.165958, 0.000000)(1.295509, 0.000000)(1.425060, 0.000000)(1.554611, 0.000000)(1.684162, 0.000000)(1.813712, 0.000000)(1.943263, 0.000000)(2.072814, 0.000000)(2.202365, 0.000000)(2.331916, 0.000000)(2.461467, 0.000000)(2.591018, 0.000000)(2.720569, 0.000000)(2.850120, 0.000000)(2.979671, 0.000000)(3.109221, 0.000000)(3.238772, 0.000000)(3.368323, 0.000000)(3.497874, 0.000000)(3.627425, 0.000000)(3.756976, 0.000000)(3.886527, 0.000000)(4.016078, 0.000000)(4.145629, 0.000000)(4.275179, 0.000000)(4.404730, 0.000000)(4.534281, 0.000000)(4.663832, 0.000000)(4.793383, 0.000000)(4.922934, 0.000000)(5.052485, 0.000000)(5.182036, 0.000000)(5.311587, 0.000000)(5.441137, 0.000000)(5.570688, 0.000000)(5.700239, 0.000000)(5.829790, 0.000000)(5.959341, 0.000000)(6.088892, 0.000000)(6.218443, 0.02)(6.347994, 0.000000)(6.477545, 0.000000)(6.607095, 0.000000)(6.736646, 0.000000)(6.866197, 0.000000)(6.995748, 0.000000)(7.125299, 0.000000)(7.254850, 0.000000)(7.384401, 0.000000)(7.513952, 0.000000)(7.643503, 0.000000)(7.773053, 0.000000)};
%\legend{Eigenvalues of ${\bm \Phi}_c$, Eigenvalues of $\tilde{{\bm \Phi}}_c$}
%\end{axis}
%\end{tikzpicture}
%\caption{Eigenvalue distribution of ${\bm \Phi}_c$ and $\tilde{{\bm \Phi}}$ for $\sigma(t)=\sin{t}$, and {\bf Student} ($\nu=7$) mixture data with ${\bm \mu}_a=[{\bf 0}_{a-1};4;{\bf 0}_{p-a}], {\bf C}_a=(1+4(a-1)/\sqrt{p}){\bf I}_p,$ $p=4096, n=2048.$}
%\label{fig:hist_L_synthetic}
%\end{figure}

\begin{figure}
\centering
    \begin{tikzpicture}[scale=1]
    		\begin{axis}[legend pos=west, xmode = log, ymode = log, west,grid=major,xlabel={$\gamma$},ylabel={MSE},xmin=1e-5,xmax=6000,ymin=0,ymax=1.2,     xtick={1e-05,0.01,1.0,5623.413251903491},
    xticklabels={$10^{-5}$, $10^{-2}$, $1$, $10^{4}$}]
    			            \addplot[mark size=4pt,only marks,red,mark=diamond,thick]coordinates{                (1e-05,0.11638548444929284)(1.778279410038923e-05,0.11638360805571912)(3.1622776601683795e-05,0.11638027203350776)(5.623413251903491e-05,0.1163743419613166)(0.0001,0.11636380391216575)(0.00017782794100389227,0.11634508731630498)(0.00031622776601683794,0.11631187647299651)(0.0005623413251903491,0.11625304655357692)(0.001,0.1161491461027549)(0.0017782794100389228,0.1159666117970721)(0.0031622776601683794,0.11564888328686715)(0.005623413251903491,0.11510462203701646)(0.01,0.11419739609924393)(0.01778279410038923,0.11275175790913991)(0.03162277660168379,0.11060643174201074)(0.05623413251903491,0.1077431749800669)(0.1,0.1044517049151024)(0.1778279410038923,0.10138088188269612)(0.31622776601683794,0.09936104103030752)(0.5623413251903491,0.09913280941506174)(1.0,0.10133492668942312)(1.7782794100389228,0.10709553378309156)(3.1622776601683795,0.1192890781414395)(5.623413251903491,0.14407307733492944)(10.0,0.19155580726538354)(17.78279410038923,0.27289600714889334)(31.622776601683793,0.39146544125829386)(56.23413251903491,0.5336319406292073)(100.0,0.6729554491313149)(177.82794100389228,0.7872317288039331)(316.22776601683796,0.8689866144983585)(562.341325190349,0.9222166794254382)(1000.0,0.9548527928141581)(1778.2794100389228,0.9741462539892911)(3162.2776601683795,0.9853102238383783)(5623.413251903491,0.9916908187874821)
};
    			            \addplot[thick,blue,only marks, mark=star, smooth]coordinates{ (1e-05,0.14377810693276755)(1.778279410038923e-05,0.14377630817106063)(3.1622776601683795e-05,0.14377310995196815)(5.623413251903491e-05,0.14376742413903482)(0.0001,0.14375731797122074)(0.00017782794100389227,0.14373936151265668)(0.00031622776601683794,0.14370747770722803)(0.0005623413251903491,0.14365092996303658)(0.001,0.14355084570151894)(0.0017782794100389228,0.14337434908963184)(0.0031622776601683794,0.1430650864147941)(0.005623413251903491,0.14252920046061857)(0.01,0.14161827052444206)(0.01778279410038923,0.1401188930019528)(0.03162277660168379,0.13777614993111295)(0.05623413251903491,0.13439606715587135)(0.1,0.13004441931114208)(0.1778279410038923,0.12523812194546158)(0.31622776601683794,0.12092808741650019)(0.5623413251903491,0.11824699977166428)(1.0,0.11835145322818183)(1.7782794100389228,0.12283727922927462)(3.1622776601683795,0.13498267797843314)(5.623413251903491,0.16142865121825442)(10.0,0.21263651069034228)(17.78279410038923,0.29901069518312756)(31.622776601683793,0.42133624377093026)(56.23413251903491,0.5631356413270733)(100.0,0.6977532219795052)(177.82794100389228,0.8053900108599666)(316.22776601683796,0.8810120829649649)(562.341325190349,0.9296713351490408)(1000.0,0.9592893838490464)(1778.2794100389228,0.9767235708951162)(3162.2776601683795,0.9867865960924078)(5623.413251903491,0.992529774200978)
};
\addplot[thick,red,smooth]coordinates{
(1e-05,0.09677305920673758)(1.778279410038923e-05,0.09696022466053268)(3.1622776601683795e-05,0.09479845298462776)(5.623413251903491e-05,0.09504658887453273)(0.0001,0.09717920451113227)(0.00017782794100389227,0.09697692581250812)(0.00031622776601683794,0.09485827912156211)(0.0005623413251903491,0.09569860343255304)(0.001,0.09210604329557874)(0.0017782794100389228,0.0924153714295605)(0.0031622776601683794,0.09058975413628141)(0.005623413251903491,0.09007153723418748)(0.01,0.08661862373981406)(0.01778279410038923,0.08317978095070602)(0.03162277660168379,0.0805227019967575)(0.05623413251903491,0.07654701880616976)(0.1,0.07507463218624293)(0.1778279410038923,0.07354087135550126)(0.31622776601683794,0.07471016019669309)(0.5623413251903491,0.07823117341112222)(1.0,0.08325553629997257)(1.7782794100389228,0.09180849495311699)(3.1622776601683795,0.10657081055647341)(5.623413251903491,0.13022282558559703)(10.0,0.16509100823880477)(17.78279410038923,0.22998842044289422)(31.622776601683793,0.3233537339424323)(56.23413251903491,0.4375297010139374)(100.0,0.5936455007840324)(177.82794100389228,0.7203199940806804)(316.22776601683796,0.8238585393646034)(562.341325190349,0.8917232432098174)(1000.0,0.9332370465044191)(1778.2794100389228,0.9630824763940741)(3162.2776601683795,0.9784979289344439)(5623.413251903491,0.9874936090021675)};
\addplot[thick,blue,smooth]coordinates{
(1e-05,0.1213441722485025)(1.778279410038923e-05,0.12515726003408081)(3.1622776601683795e-05,0.12287233468432902)(5.623413251903491e-05,0.12318514382269966)(0.0001,0.12363033512178849)(0.00017782794100389227,0.12125433808773002)(0.00031622776601683794,0.12382500566683387)(0.0005623413251903491,0.12270216131342561)(0.001,0.1210672186029946)(0.0017782794100389228,0.12205271637548383)(0.0031622776601683794,0.12017739765700129)(0.005623413251903491,0.11760523734477672)(0.01,0.11838840366805561)(0.01778279410038923,0.11581169262590059)(0.03162277660168379,0.11364949903629444)(0.05623413251903491,0.10614961869432898)(0.1,0.10290124763731448)(0.1778279410038923,0.09750279087432785)(0.31622776601683794,0.09673542755294219)(0.5623413251903491,0.09834522939407057)(1.0,0.1044442420934261)(1.7782794100389228,0.11485824390741158)(3.1622776601683795,0.13863764994583005)(5.623413251903491,0.1773183478700117)(10.0,0.24315466201301794)(17.78279410038923,0.3476317437947627)(31.622776601683793,0.48467618098856946)(56.23413251903491,0.6239343526077076)(100.0,0.7514529638783835)(177.82794100389228,0.8429822148517248)(316.22776601683796,0.9066549861233849)(562.341325190349,0.9459773093638947)(1000.0,0.9683763513256203)(1778.2794100389228,0.9825307337796058)(3162.2776601683795,0.9899386625708262)(5623.413251903491,0.9943234690259272)};
\legend{(ReLU Th),(Ternary Th), (ReLU Emp),(Ternary Emp)};
    		\end{axis}
    \end{tikzpicture}
\caption{Testing MSE of kernel ridge regression as a function of regularization parameter $\gamma,$ $p=784, n=512, \hat{n}=256, m=128.$ ReLU activation function versus Ternary function (with thresholds $s_1, s_2$ chosen to match gaussian moments of ReLU). Fashion MNIST}
\label{fig:compare_relu_ternary}
\end{figure}

